Unveiling the shape of the $^{20}$Ne nucleus by measuring the flow coefficients with cumulants in PbNe and PbAr collisions at $\sqrt{s_{NN}} = 70.9$ GeV

The anisotropic flow coefficients $v_n$ quantify the collective medium response to the initial spatial anisotropy of the overlapping region in ion collisions and serve as sensitive probes of both the medium properties and shape of nuclear initial states. In this analysis, the $v_2$ and $v_3$ parameters of prompt charged particles are measured using the multiparticle cumulant method in fixed-target PbNe and PbAr collisions at $\sqrt{s_{NN}} = 70.9$ GeV, collected by LHCb using the SMOG2 gas-target system during the 2024 LHC lead-beam run. The cumulant method is first validated using 2018 PbPb collision data, successfully reproducing previous measurements obtained via the two-particle correlation method. Results for the fixed-target collisions are then presented, showing a significantly larger value of the elliptic flow coefficient $v_2$ in central PbNe with respect to PbAr collisions. This is qualitatively consistent with 3+1D hydrodynamic predictions including ab-initio descriptions of the nuclear structure. The results provide the first experimental confirmation of the distinctive bowling-pin shape of the ground-state $^{20}$Ne nucleus, validating at the same time the hydrodynamic description of the hot medium formed in high-energy collisions involving light ions.

==> Authorship_LHCb-CONF-2025-001-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
M.  Akthar,
P. Albicocco,
J. Albrecht,
R.  Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
P. Andreola,
M. Andreotti,
S.  Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L.  Arnone,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ata\'{i}de Da Silva,
M. Atzeni,
B. Audurier,
J. A.  Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
A.  Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H.  Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P. B.  Battista,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N. A.  Behling,
S. Belin,
A.  Bellavista,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
F. Betti,
J.  Bex,
O. Bezshyyko,
S.  Bhattacharya,
J. Bhom,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C.S. Bolognani,
R. Bolzonella,
R. B.  Bonacci,
N. Bondar,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E.  Bottalico,
S.A. Bouchiba,
M.  Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J. D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
J. Brown,
D. Brundu,
E. Buchanan,
M.  Burgos Marcos,
A.T. Burke,
C. Burr,
C.  Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y.  Cai,
A. Caillet,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
A.F. Campoverde Quezada,
S. Capelli,
M.  Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I.  Celestino,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
H.  Chang,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
R.  Cheaib,
M. Chefdeville,
C. Chen,
J.  Chen,
S. Chen,
Z. Chen,
A.  Chen Hu,
M.  Cherif,
A. Chernov,
S. Chernyshenko,
X.  Chiotopoulos,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S.  Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J.  Connaughton,
A. Contu,
N. Cooke,
G. Cordova,
C.  Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
G. Darze,
A.  Davidson,
J.E. Davies,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S.  Dekkers,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
Y.  Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
A.  Doheny,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D.  Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
S.  Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K.   Farmer,
F.  Fassin,
D. Fazzini,
L. Felkowski,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.L. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A.  Fomin,
M. Fontana,
L. F.  Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. F{\"u}hring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
P.  Gardner,
L. Garrido,
C. Gaspar,
A.  Gavrikov,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
L.  Golinka-Bezshyyko,
E. Golobardes,
D. Golubkov,
A. Golutvin,
S. Gomez Fernandez,
W.  Gomulka,
I. Gonçales Vaz,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
L.  Guerry,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.  Haken,
G.  Hallett,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
T. H.  Harris,
M. Hartmann,
S. Hashmi,
J. He,
N.  Heatley,
A.  Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A.  Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D. C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
M. Idzik,
D. Ilin,
P. Ilten,
A. Iniukhin,
A.  Iohner,
A. Ishteev,
K. Ivshin,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
B.K. Jashal,
A. Jawahery,
C.  Jayaweera,
V. Jevtic,
Z.  Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
E. Jimenez Moya,
N.  Jindal,
M. John,
A.  John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J.  Juan Castella,
N. Jurik,
I. Juszczak,
K.  Kalecinska,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
S. Klaver,
N. Kleijne,
A. Kleimenova,
D. K.  Klekots,
K. Klimaszewski,
M.R. Kmiec,
T.  Knospe,
R.  Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
A.  Korchin,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E.  Kowalczyk,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
O.  Kravcov,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I.  Kyryllin,
D. Lacarrere,
P.  Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H.  Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E. D. Lesser,
B. Leverington,
A. Li,
C.  Li,
C.  Li,
H. Li,
J. Li,
K. Li,
L. Li,
M. Li,
P. Li,
P.-R. Li,
Q.  Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Y.  Li,
Z. Lian,
Q.  Liang,
X. Liang,
Z.  Liang,
S. Libralon,
A. L.  Lightbody,
C. Lin,
T. Lin,
R. Lindner,
H.  Linton,
R. Litvinov,
D. Liu,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
W.  Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
G. Loachamin Ordonez,
I.  Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F. C. L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C.  Lopez Iribarnegaray,
S. L{\'o}pez Soli{\~n}o,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
H.  Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. J.  Madurai,
D. Magdalinski,
D. Maisuzenko,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
F. M.  Manganella,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L.  Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D.  Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A.  Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
D. Mendoza Granada,
P.  Menendez Valdes Perez,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
R.  Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E. F. Molina Cardenas,
T. Momb{\"a}cher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A.  Moro,
J. Moron,
W.  Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
V.  Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
G.  Napoletano,
I. Nasteva,
M. Needham,
E.  Nekrasova,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
L.  Nisi,
Q. Niu,
P. Nogarolli,
P. Nogga,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E.  Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A.  Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L.  Palini,
M. Palutan,
C.  Pan,
X.  Pan,
S. Panebianco,
S. Paniskaki,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D.  Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
X.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
M.  Pereira Martinez,
A. Pereiro Castro,
C.  Perez,
P. Perret,
A.  Perrevoort,
A. Perro,
M.J. Peters,
K. Petridis,
A. Petrolini,
S.  Pezzulo,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L.  Piccolo,
B. Pietrzyk,
G. Pietrzyk,
R. N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
S. Poslavskii,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A.  Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Q.  Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
R.  Racz,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M.  Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F.  Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogachev,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
S. E. R. Sacha Emile R.,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G.  Scriven,
I. Segal,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
B.  Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
W. S.  Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
M.  Singha,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
K. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
K.  Solovieva,
N. S.  Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M.  Stefaniak,
E.N. Stein,
O. Steinkamp,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
J.  Sun,
L. Sun,
D. Sundfeld,
W. Sutcliffe,
P. Svihra,
V. Svintozelskyi,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y. T.  Tang,
M.D. Tat,
J. A. Teijeiro Jimenez,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A. R.  Thomson-Strong,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T. T.  Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
A.  Upadhyay,
B.  Urbach,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
A.  Vaitkevicius,
V.  Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.  Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D.  Vico Benet,
P.  Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
A.  Wang,
B.  Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Y. Wang,
Y. H.  Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z.  Weida,
J. Wendel,
B.D.C. Westhenry,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M. A. Wiegertjes,
C.  Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M. J. Williams,
M.R.J. Williams,
R. Williams,
S.  Williams,
Z.  Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E.  Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T. X.  Xing,
A. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S.  Yadav,
K.  Yang,
X. Yang,
Y. Yang,
Y.  Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
X.  Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
Y Yuan,
J. A. Zamora Saa,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
R. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Z.  Zhang,
Z. Zhang,
Y. Zhao,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
Y.  Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
D. Zuliani,
G. Zunica

==> Authorship_LHCb-CONF-2025-001.tex <==
% LHCb collaboration author list
% Data extracted on September 12th, 2025 at 3:12pm for paper reference LHCb-CONF-2025-001
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{38}$\lhcborcid{0000-0003-0533-1952},
A.S.W.~Abdelmotteleb$^{58}$\lhcborcid{0000-0001-7905-0542},
C.~Abellan~Beteta$^{52}$\lhcborcid{0009-0009-0869-6798},
F.~Abudin{\'e}n$^{58}$\lhcborcid{0000-0002-6737-3528},
T.~Ackernley$^{62}$\lhcborcid{0000-0002-5951-3498},
A. A. ~Adefisoye$^{70}$\lhcborcid{0000-0003-2448-1550},
B.~Adeva$^{48}$\lhcborcid{0000-0001-9756-3712},
M.~Adinolfi$^{56}$\lhcborcid{0000-0002-1326-1264},
P.~Adlarson$^{86}$\lhcborcid{0000-0001-6280-3851},
C.~Agapopoulou$^{14}$\lhcborcid{0000-0002-2368-0147},
C.A.~Aidala$^{88}$\lhcborcid{0000-0001-9540-4988},
Z.~Ajaltouni$^{11}$,
S.~Akar$^{11}$\lhcborcid{0000-0003-0288-9694},
K.~Akiba$^{38}$\lhcborcid{0000-0002-6736-471X},
M. ~Akthar$^{40}$\lhcborcid{0009-0003-3172-2997},
P.~Albicocco$^{28}$\lhcborcid{0000-0001-6430-1038},
J.~Albrecht$^{19,g}$\lhcborcid{0000-0001-8636-1621},
R. ~Aleksiejunas$^{82}$\lhcborcid{0000-0002-9093-2252},
F.~Alessio$^{50}$\lhcborcid{0000-0001-5317-1098},
P.~Alvarez~Cartelle$^{57,48}$\lhcborcid{0000-0003-1652-2834},
R.~Amalric$^{16}$\lhcborcid{0000-0003-4595-2729},
S.~Amato$^{3}$\lhcborcid{0000-0002-3277-0662},
J.L.~Amey$^{56}$\lhcborcid{0000-0002-2597-3808},
Y.~Amhis$^{14}$\lhcborcid{0000-0003-4282-1512},
L.~An$^{6}$\lhcborcid{0000-0002-3274-5627},
L.~Anderlini$^{27}$\lhcborcid{0000-0001-6808-2418},
M.~Andersson$^{52}$\lhcborcid{0000-0003-3594-9163},
P.~Andreola$^{52}$\lhcborcid{0000-0002-3923-431X},
M.~Andreotti$^{26}$\lhcborcid{0000-0003-2918-1311},
S. ~Andres~Estrada$^{45}$\lhcborcid{0009-0004-1572-0964},
A.~Anelli$^{31,p,50}$\lhcborcid{0000-0002-6191-934X},
D.~Ao$^{7}$\lhcborcid{0000-0003-1647-4238},
C.~Arata$^{12}$\lhcborcid{0009-0002-1990-7289},
F.~Archilli$^{37,v}$\lhcborcid{0000-0002-1779-6813},
Z.~Areg$^{70}$\lhcborcid{0009-0001-8618-2305},
M.~Argenton$^{26}$\lhcborcid{0009-0006-3169-0077},
S.~Arguedas~Cuendis$^{9,50}$\lhcborcid{0000-0003-4234-7005},
L. ~Arnone$^{31,p}$\lhcborcid{0009-0008-2154-8493},
A.~Artamonov$^{44}$\lhcborcid{0000-0002-2785-2233},
M.~Artuso$^{70}$\lhcborcid{0000-0002-5991-7273},
E.~Aslanides$^{13}$\lhcborcid{0000-0003-3286-683X},
R.~Ata\'{i}de~Da~Silva$^{51}$\lhcborcid{0009-0005-1667-2666},
M.~Atzeni$^{66}$\lhcborcid{0000-0002-3208-3336},
B.~Audurier$^{12}$\lhcborcid{0000-0001-9090-4254},
J. A. ~Authier$^{15}$\lhcborcid{0009-0000-4716-5097},
D.~Bacher$^{65}$\lhcborcid{0000-0002-1249-367X},
I.~Bachiller~Perea$^{51}$\lhcborcid{0000-0002-3721-4876},
S.~Bachmann$^{22}$\lhcborcid{0000-0002-1186-3894},
M.~Bachmayer$^{51}$\lhcborcid{0000-0001-5996-2747},
J.J.~Back$^{58}$\lhcborcid{0000-0001-7791-4490},
P.~Baladron~Rodriguez$^{48}$\lhcborcid{0000-0003-4240-2094},
V.~Balagura$^{15}$\lhcborcid{0000-0002-1611-7188},
A. ~Balboni$^{26}$\lhcborcid{0009-0003-8872-976X},
W.~Baldini$^{26}$\lhcborcid{0000-0001-7658-8777},
Z.~Baldwin$^{80}$\lhcborcid{0000-0002-8534-0922},
L.~Balzani$^{19}$\lhcborcid{0009-0006-5241-1452},
H. ~Bao$^{7}$\lhcborcid{0009-0002-7027-021X},
J.~Baptista~de~Souza~Leite$^{2}$\lhcborcid{0000-0002-4442-5372},
C.~Barbero~Pretel$^{48,12}$\lhcborcid{0009-0001-1805-6219},
M.~Barbetti$^{27}$\lhcborcid{0000-0002-6704-6914},
I. R.~Barbosa$^{71}$\lhcborcid{0000-0002-3226-8672},
R.J.~Barlow$^{64}$\lhcborcid{0000-0002-8295-8612},
M.~Barnyakov$^{25}$\lhcborcid{0009-0000-0102-0482},
S.~Barsuk$^{14}$\lhcborcid{0000-0002-0898-6551},
W.~Barter$^{60}$\lhcborcid{0000-0002-9264-4799},
J.~Bartz$^{70}$\lhcborcid{0000-0002-2646-4124},
S.~Bashir$^{40}$\lhcborcid{0000-0001-9861-8922},
B.~Batsukh$^{5}$\lhcborcid{0000-0003-1020-2549},
P. B. ~Battista$^{14}$\lhcborcid{0009-0005-5095-0439},
A.~Bay$^{51}$\lhcborcid{0000-0002-4862-9399},
A.~Beck$^{66}$\lhcborcid{0000-0003-4872-1213},
M.~Becker$^{19}$\lhcborcid{0000-0002-7972-8760},
F.~Bedeschi$^{35}$\lhcborcid{0000-0002-8315-2119},
I.B.~Bediaga$^{2}$\lhcborcid{0000-0001-7806-5283},
N. A. ~Behling$^{19}$\lhcborcid{0000-0003-4750-7872},
S.~Belin$^{48}$\lhcborcid{0000-0001-7154-1304},
A. ~Bellavista$^{25}$\lhcborcid{0009-0009-3723-834X},
K.~Belous$^{44}$\lhcborcid{0000-0003-0014-2589},
I.~Belov$^{29}$\lhcborcid{0000-0003-1699-9202},
I.~Belyaev$^{36}$\lhcborcid{0000-0002-7458-7030},
G.~Benane$^{13}$\lhcborcid{0000-0002-8176-8315},
G.~Bencivenni$^{28}$\lhcborcid{0000-0002-5107-0610},
E.~Ben-Haim$^{16}$\lhcborcid{0000-0002-9510-8414},
A.~Berezhnoy$^{44}$\lhcborcid{0000-0002-4431-7582},
R.~Bernet$^{52}$\lhcborcid{0000-0002-4856-8063},
S.~Bernet~Andres$^{47}$\lhcborcid{0000-0002-4515-7541},
A.~Bertolin$^{33}$\lhcborcid{0000-0003-1393-4315},
F.~Betti$^{60}$\lhcborcid{0000-0002-2395-235X},
J. ~Bex$^{57}$\lhcborcid{0000-0002-2856-8074},
O.~Bezshyyko$^{87}$\lhcborcid{0000-0001-7106-5213},
S. ~Bhattacharya$^{81}$\lhcborcid{0009-0007-8372-6008},
J.~Bhom$^{41}$\lhcborcid{0000-0002-9709-903X},
M.S.~Bieker$^{18}$\lhcborcid{0000-0001-7113-7862},
N.V.~Biesuz$^{26}$\lhcborcid{0000-0003-3004-0946},
A.~Biolchini$^{38}$\lhcborcid{0000-0001-6064-9993},
M.~Birch$^{63}$\lhcborcid{0000-0001-9157-4461},
F.C.R.~Bishop$^{10}$\lhcborcid{0000-0002-0023-3897},
A.~Bitadze$^{64}$\lhcborcid{0000-0001-7979-1092},
A.~Bizzeti$^{27,q}$\lhcborcid{0000-0001-5729-5530},
T.~Blake$^{58,c}$\lhcborcid{0000-0002-0259-5891},
F.~Blanc$^{51}$\lhcborcid{0000-0001-5775-3132},
J.E.~Blank$^{19}$\lhcborcid{0000-0002-6546-5605},
S.~Blusk$^{70}$\lhcborcid{0000-0001-9170-684X},
V.~Bocharnikov$^{44}$\lhcborcid{0000-0003-1048-7732},
J.A.~Boelhauve$^{19}$\lhcborcid{0000-0002-3543-9959},
O.~Boente~Garcia$^{50}$\lhcborcid{0000-0003-0261-8085},
T.~Boettcher$^{69}$\lhcborcid{0000-0002-2439-9955},
A. ~Bohare$^{60}$\lhcborcid{0000-0003-1077-8046},
A.~Boldyrev$^{44}$\lhcborcid{0000-0002-7872-6819},
C.S.~Bolognani$^{84}$\lhcborcid{0000-0003-3752-6789},
R.~Bolzonella$^{26,m}$\lhcborcid{0000-0002-0055-0577},
R. B. ~Bonacci$^{1}$\lhcborcid{0009-0004-1871-2417},
N.~Bondar$^{44,50}$\lhcborcid{0000-0003-2714-9879},
A.~Bordelius$^{50}$\lhcborcid{0009-0002-3529-8524},
F.~Borgato$^{33,50}$\lhcborcid{0000-0002-3149-6710},
S.~Borghi$^{64}$\lhcborcid{0000-0001-5135-1511},
M.~Borsato$^{31,p}$\lhcborcid{0000-0001-5760-2924},
J.T.~Borsuk$^{85}$\lhcborcid{0000-0002-9065-9030},
E. ~Bottalico$^{62}$\lhcborcid{0000-0003-2238-8803},
S.A.~Bouchiba$^{51}$\lhcborcid{0000-0002-0044-6470},
M. ~Bovill$^{65}$\lhcborcid{0009-0006-2494-8287},
T.J.V.~Bowcock$^{62}$\lhcborcid{0000-0002-3505-6915},
A.~Boyer$^{50}$\lhcborcid{0000-0002-9909-0186},
C.~Bozzi$^{26}$\lhcborcid{0000-0001-6782-3982},
J. D.~Brandenburg$^{89}$\lhcborcid{0000-0002-6327-5947},
A.~Brea~Rodriguez$^{51}$\lhcborcid{0000-0001-5650-445X},
N.~Breer$^{19}$\lhcborcid{0000-0003-0307-3662},
J.~Brodzicka$^{41}$\lhcborcid{0000-0002-8556-0597},
J.~Brown$^{62}$\lhcborcid{0000-0001-9846-9672},
D.~Brundu$^{32}$\lhcborcid{0000-0003-4457-5896},
E.~Buchanan$^{60}$\lhcborcid{0009-0008-3263-1823},
M. ~Burgos~Marcos$^{84}$\lhcborcid{0009-0001-9716-0793},
A.T.~Burke$^{64}$\lhcborcid{0000-0003-0243-0517},
C.~Burr$^{50}$\lhcborcid{0000-0002-5155-1094},
C. ~Buti$^{27}$\lhcborcid{0009-0009-2488-5548},
J.S.~Butter$^{57}$\lhcborcid{0000-0002-1816-536X},
J.~Buytaert$^{50}$\lhcborcid{0000-0002-7958-6790},
W.~Byczynski$^{50}$\lhcborcid{0009-0008-0187-3395},
S.~Cadeddu$^{32}$\lhcborcid{0000-0002-7763-500X},
H.~Cai$^{76}$\lhcborcid{0000-0003-0898-3673},
Y. ~Cai$^{5}$\lhcborcid{0009-0004-5445-9404},
A.~Caillet$^{16}$\lhcborcid{0009-0001-8340-3870},
R.~Calabrese$^{26,m}$\lhcborcid{0000-0002-1354-5400},
S.~Calderon~Ramirez$^{9}$\lhcborcid{0000-0001-9993-4388},
L.~Calefice$^{46}$\lhcborcid{0000-0001-6401-1583},
M.~Calvi$^{31,p}$\lhcborcid{0000-0002-8797-1357},
M.~Calvo~Gomez$^{47}$\lhcborcid{0000-0001-5588-1448},
P.~Camargo~Magalhaes$^{2,a}$\lhcborcid{0000-0003-3641-8110},
J. I.~Cambon~Bouzas$^{48}$\lhcborcid{0000-0002-2952-3118},
P.~Campana$^{28}$\lhcborcid{0000-0001-8233-1951},
A.F.~Campoverde~Quezada$^{7}$\lhcborcid{0000-0003-1968-1216},
S.~Capelli$^{31}$\lhcborcid{0000-0002-8444-4498},
M. ~Caporale$^{25}$\lhcborcid{0009-0008-9395-8723},
L.~Capriotti$^{26}$\lhcborcid{0000-0003-4899-0587},
R.~Caravaca-Mora$^{9}$\lhcborcid{0000-0001-8010-0447},
A.~Carbone$^{25,k}$\lhcborcid{0000-0002-7045-2243},
L.~Carcedo~Salgado$^{48}$\lhcborcid{0000-0003-3101-3528},
R.~Cardinale$^{29,n}$\lhcborcid{0000-0002-7835-7638},
A.~Cardini$^{32}$\lhcborcid{0000-0002-6649-0298},
P.~Carniti$^{31}$\lhcborcid{0000-0002-7820-2732},
L.~Carus$^{22}$\lhcborcid{0009-0009-5251-2474},
A.~Casais~Vidal$^{66}$\lhcborcid{0000-0003-0469-2588},
R.~Caspary$^{22}$\lhcborcid{0000-0002-1449-1619},
G.~Casse$^{62}$\lhcborcid{0000-0002-8516-237X},
M.~Cattaneo$^{50}$\lhcborcid{0000-0001-7707-169X},
G.~Cavallero$^{26}$\lhcborcid{0000-0002-8342-7047},
V.~Cavallini$^{26,m}$\lhcborcid{0000-0001-7601-129X},
S.~Celani$^{50}$\lhcborcid{0000-0003-4715-7622},
I. ~Celestino$^{35,t}$\lhcborcid{0009-0008-0215-0308},
S. ~Cesare$^{30,o}$\lhcborcid{0000-0003-0886-7111},
A.J.~Chadwick$^{62}$\lhcborcid{0000-0003-3537-9404},
I.~Chahrour$^{88}$\lhcborcid{0000-0002-1472-0987},
H. ~Chang$^{4,d}$\lhcborcid{0009-0002-8662-1918},
M.~Charles$^{16}$\lhcborcid{0000-0003-4795-498X},
Ph.~Charpentier$^{50}$\lhcborcid{0000-0001-9295-8635},
E. ~Chatzianagnostou$^{38}$\lhcborcid{0009-0009-3781-1820},
R. ~Cheaib$^{81}$\lhcborcid{0000-0002-6292-3068},
M.~Chefdeville$^{10}$\lhcborcid{0000-0002-6553-6493},
C.~Chen$^{57}$\lhcborcid{0000-0002-3400-5489},
J. ~Chen$^{51}$\lhcborcid{0009-0006-1819-4271},
S.~Chen$^{5}$\lhcborcid{0000-0002-8647-1828},
Z.~Chen$^{7}$\lhcborcid{0000-0002-0215-7269},
A. ~Chen~Hu$^{63}$\lhcborcid{0009-0002-3626-8909 },
M. ~Cherif$^{12}$\lhcborcid{0009-0004-4839-7139},
A.~Chernov$^{41}$\lhcborcid{0000-0003-0232-6808},
S.~Chernyshenko$^{54}$\lhcborcid{0000-0002-2546-6080},
X. ~Chiotopoulos$^{84}$\lhcborcid{0009-0006-5762-6559},
V.~Chobanova$^{45}$\lhcborcid{0000-0002-1353-6002},
M.~Chrzaszcz$^{41}$\lhcborcid{0000-0001-7901-8710},
A.~Chubykin$^{44}$\lhcborcid{0000-0003-1061-9643},
V.~Chulikov$^{28,36,50}$\lhcborcid{0000-0002-7767-9117},
P.~Ciambrone$^{28}$\lhcborcid{0000-0003-0253-9846},
X.~Cid~Vidal$^{48}$\lhcborcid{0000-0002-0468-541X},
G.~Ciezarek$^{50}$\lhcborcid{0000-0003-1002-8368},
P.~Cifra$^{38}$\lhcborcid{0000-0003-3068-7029},
P.E.L.~Clarke$^{60}$\lhcborcid{0000-0003-3746-0732},
M.~Clemencic$^{50}$\lhcborcid{0000-0003-1710-6824},
H.V.~Cliff$^{57}$\lhcborcid{0000-0003-0531-0916},
J.~Closier$^{50}$\lhcborcid{0000-0002-0228-9130},
C.~Cocha~Toapaxi$^{22}$\lhcborcid{0000-0001-5812-8611},
V.~Coco$^{50}$\lhcborcid{0000-0002-5310-6808},
J.~Cogan$^{13}$\lhcborcid{0000-0001-7194-7566},
E.~Cogneras$^{11}$\lhcborcid{0000-0002-8933-9427},
L.~Cojocariu$^{43}$\lhcborcid{0000-0002-1281-5923},
S. ~Collaviti$^{51}$\lhcborcid{0009-0003-7280-8236},
P.~Collins$^{50}$\lhcborcid{0000-0003-1437-4022},
T.~Colombo$^{50}$\lhcborcid{0000-0002-9617-9687},
M.~Colonna$^{19}$\lhcborcid{0009-0000-1704-4139},
A.~Comerma-Montells$^{46}$\lhcborcid{0000-0002-8980-6048},
L.~Congedo$^{24}$\lhcborcid{0000-0003-4536-4644},
J. ~Connaughton$^{58}$\lhcborcid{0000-0003-2557-4361},
A.~Contu$^{32}$\lhcborcid{0000-0002-3545-2969},
N.~Cooke$^{61}$\lhcborcid{0000-0002-4179-3700},
G.~Cordova$^{35,t}$\lhcborcid{0009-0003-8308-4798},
C. ~Coronel$^{67}$\lhcborcid{0009-0006-9231-4024},
I.~Corredoira~$^{12}$\lhcborcid{0000-0002-6089-0899},
A.~Correia$^{16}$\lhcborcid{0000-0002-6483-8596},
G.~Corti$^{50}$\lhcborcid{0000-0003-2857-4471},
J.~Cottee~Meldrum$^{56}$\lhcborcid{0009-0009-3900-6905},
B.~Couturier$^{50}$\lhcborcid{0000-0001-6749-1033},
D.C.~Craik$^{52}$\lhcborcid{0000-0002-3684-1560},
M.~Cruz~Torres$^{2,h}$\lhcborcid{0000-0003-2607-131X},
E.~Curras~Rivera$^{51}$\lhcborcid{0000-0002-6555-0340},
R.~Currie$^{60}$\lhcborcid{0000-0002-0166-9529},
C.L.~Da~Silva$^{69}$\lhcborcid{0000-0003-4106-8258},
S.~Dadabaev$^{44}$\lhcborcid{0000-0002-0093-3244},
X.~Dai$^{4}$\lhcborcid{0000-0003-3395-7151},
E.~Dall'Occo$^{50}$\lhcborcid{0000-0001-9313-4021},
J.~Dalseno$^{45}$\lhcborcid{0000-0003-3288-4683},
C.~D'Ambrosio$^{63}$\lhcborcid{0000-0003-4344-9994},
J.~Daniel$^{11}$\lhcborcid{0000-0002-9022-4264},
G.~Darze$^{3}$\lhcborcid{0000-0002-7666-6533},
A. ~Davidson$^{58}$\lhcborcid{0009-0002-0647-2028},
J.E.~Davies$^{64}$\lhcborcid{0000-0002-5382-8683},
O.~De~Aguiar~Francisco$^{64}$\lhcborcid{0000-0003-2735-678X},
C.~De~Angelis$^{32,l}$\lhcborcid{0009-0005-5033-5866},
F.~De~Benedetti$^{50}$\lhcborcid{0000-0002-7960-3116},
J.~de~Boer$^{38}$\lhcborcid{0000-0002-6084-4294},
K.~De~Bruyn$^{83}$\lhcborcid{0000-0002-0615-4399},
S.~De~Capua$^{64}$\lhcborcid{0000-0002-6285-9596},
M.~De~Cian$^{64,50}$\lhcborcid{0000-0002-1268-9621},
U.~De~Freitas~Carneiro~Da~Graca$^{2,b}$\lhcborcid{0000-0003-0451-4028},
E.~De~Lucia$^{28}$\lhcborcid{0000-0003-0793-0844},
J.M.~De~Miranda$^{2}$\lhcborcid{0009-0003-2505-7337},
L.~De~Paula$^{3}$\lhcborcid{0000-0002-4984-7734},
M.~De~Serio$^{24,i}$\lhcborcid{0000-0003-4915-7933},
P.~De~Simone$^{28}$\lhcborcid{0000-0001-9392-2079},
F.~De~Vellis$^{19}$\lhcborcid{0000-0001-7596-5091},
J.A.~de~Vries$^{84}$\lhcborcid{0000-0003-4712-9816},
F.~Debernardis$^{24}$\lhcborcid{0009-0001-5383-4899},
D.~Decamp$^{10}$\lhcborcid{0000-0001-9643-6762},
S. ~Dekkers$^{1}$\lhcborcid{0000-0001-9598-875X},
L.~Del~Buono$^{16}$\lhcborcid{0000-0003-4774-2194},
B.~Delaney$^{66}$\lhcborcid{0009-0007-6371-8035},
H.-P.~Dembinski$^{19}$\lhcborcid{0000-0003-3337-3850},
J.~Deng$^{8}$\lhcborcid{0000-0002-4395-3616},
V.~Denysenko$^{52}$\lhcborcid{0000-0002-0455-5404},
O.~Deschamps$^{11}$\lhcborcid{0000-0002-7047-6042},
F.~Dettori$^{32,l}$\lhcborcid{0000-0003-0256-8663},
B.~Dey$^{81}$\lhcborcid{0000-0002-4563-5806},
P.~Di~Nezza$^{28}$\lhcborcid{0000-0003-4894-6762},
I.~Diachkov$^{44}$\lhcborcid{0000-0001-5222-5293},
S.~Didenko$^{44}$\lhcborcid{0000-0001-5671-5863},
S.~Ding$^{70}$\lhcborcid{0000-0002-5946-581X},
Y. ~Ding$^{51}$\lhcborcid{0009-0008-2518-8392},
L.~Dittmann$^{22}$\lhcborcid{0009-0000-0510-0252},
V.~Dobishuk$^{54}$\lhcborcid{0000-0001-9004-3255},
A. D. ~Docheva$^{61}$\lhcborcid{0000-0002-7680-4043},
A. ~Doheny$^{58}$\lhcborcid{0009-0006-2410-6282},
C.~Dong$^{4,d}$\lhcborcid{0000-0003-3259-6323},
A.M.~Donohoe$^{23}$\lhcborcid{0000-0002-4438-3950},
F.~Dordei$^{32}$\lhcborcid{0000-0002-2571-5067},
A.C.~dos~Reis$^{2}$\lhcborcid{0000-0001-7517-8418},
A. D. ~Dowling$^{70}$\lhcborcid{0009-0007-1406-3343},
L.~Dreyfus$^{13}$\lhcborcid{0009-0000-2823-5141},
W.~Duan$^{74}$\lhcborcid{0000-0003-1765-9939},
P.~Duda$^{85}$\lhcborcid{0000-0003-4043-7963},
L.~Dufour$^{50}$\lhcborcid{0000-0002-3924-2774},
V.~Duk$^{34}$\lhcborcid{0000-0001-6440-0087},
P.~Durante$^{50}$\lhcborcid{0000-0002-1204-2270},
M. M.~Duras$^{85}$\lhcborcid{0000-0002-4153-5293},
J.M.~Durham$^{69}$\lhcborcid{0000-0002-5831-3398},
O. D. ~Durmus$^{81}$\lhcborcid{0000-0002-8161-7832},
A.~Dziurda$^{41}$\lhcborcid{0000-0003-4338-7156},
A.~Dzyuba$^{44}$\lhcborcid{0000-0003-3612-3195},
S.~Easo$^{59}$\lhcborcid{0000-0002-4027-7333},
E.~Eckstein$^{18}$\lhcborcid{0009-0009-5267-5177},
U.~Egede$^{1}$\lhcborcid{0000-0001-5493-0762},
A.~Egorychev$^{44}$\lhcborcid{0000-0001-5555-8982},
V.~Egorychev$^{44}$\lhcborcid{0000-0002-2539-673X},
S.~Eisenhardt$^{60}$\lhcborcid{0000-0002-4860-6779},
E.~Ejopu$^{62}$\lhcborcid{0000-0003-3711-7547},
L.~Eklund$^{86}$\lhcborcid{0000-0002-2014-3864},
M.~Elashri$^{67}$\lhcborcid{0000-0001-9398-953X},
D. ~Elizondo~Blanco$^{9}$,
J.~Ellbracht$^{19}$\lhcborcid{0000-0003-1231-6347},
S.~Ely$^{63}$\lhcborcid{0000-0003-1618-3617},
A.~Ene$^{43}$\lhcborcid{0000-0001-5513-0927},
J.~Eschle$^{70}$\lhcborcid{0000-0002-7312-3699},
S.~Esen$^{22}$\lhcborcid{0000-0003-2437-8078},
T.~Evans$^{38}$\lhcborcid{0000-0003-3016-1879},
F.~Fabiano$^{32}$\lhcborcid{0000-0001-6915-9923},
S. ~Faghih$^{67}$\lhcborcid{0009-0008-3848-4967},
L.N.~Falcao$^{31,p}$\lhcborcid{0000-0003-3441-583X},
B.~Fang$^{7}$\lhcborcid{0000-0003-0030-3813},
R.~Fantechi$^{35}$\lhcborcid{0000-0002-6243-5726},
L.~Fantini$^{34,s}$\lhcborcid{0000-0002-2351-3998},
M.~Faria$^{51}$\lhcborcid{0000-0002-4675-4209},
K.  ~Farmer$^{60}$\lhcborcid{0000-0003-2364-2877},
F. ~Fassin$^{83,38}$\lhcborcid{0009-0002-9804-5364},
D.~Fazzini$^{31,p}$\lhcborcid{0000-0002-5938-4286},
L.~Felkowski$^{85}$\lhcborcid{0000-0002-0196-910X},
M.~Feng$^{5,7}$\lhcborcid{0000-0002-6308-5078},
A.~Fernandez~Casani$^{49}$\lhcborcid{0000-0003-1394-509X},
M.~Fernandez~Gomez$^{48}$\lhcborcid{0000-0003-1984-4759},
A.D.~Fernez$^{68}$\lhcborcid{0000-0001-9900-6514},
F.~Ferrari$^{25,k}$\lhcborcid{0000-0002-3721-4585},
F.~Ferreira~Rodrigues$^{3}$\lhcborcid{0000-0002-4274-5583},
M.~Ferrillo$^{52}$\lhcborcid{0000-0003-1052-2198},
M.~Ferro-Luzzi$^{50}$\lhcborcid{0009-0008-1868-2165},
S.~Filippov$^{44}$\lhcborcid{0000-0003-3900-3914},
R.A.~Fini$^{24}$\lhcborcid{0000-0002-3821-3998},
M.~Fiorini$^{26,m}$\lhcborcid{0000-0001-6559-2084},
M.~Firlej$^{40}$\lhcborcid{0000-0002-1084-0084},
K.L.~Fischer$^{65}$\lhcborcid{0009-0000-8700-9910},
D.S.~Fitzgerald$^{88}$\lhcborcid{0000-0001-6862-6876},
C.~Fitzpatrick$^{64}$\lhcborcid{0000-0003-3674-0812},
T.~Fiutowski$^{40}$\lhcborcid{0000-0003-2342-8854},
F.~Fleuret$^{15}$\lhcborcid{0000-0002-2430-782X},
A. ~Fomin$^{53}$\lhcborcid{0000-0002-3631-0604},
M.~Fontana$^{25}$\lhcborcid{0000-0003-4727-831X},
L. F. ~Foreman$^{64}$\lhcborcid{0000-0002-2741-9966},
R.~Forty$^{50}$\lhcborcid{0000-0003-2103-7577},
D.~Foulds-Holt$^{60}$\lhcborcid{0000-0001-9921-687X},
V.~Franco~Lima$^{3}$\lhcborcid{0000-0002-3761-209X},
M.~Franco~Sevilla$^{68}$\lhcborcid{0000-0002-5250-2948},
M.~Frank$^{50}$\lhcborcid{0000-0002-4625-559X},
E.~Franzoso$^{26,m}$\lhcborcid{0000-0003-2130-1593},
G.~Frau$^{64}$\lhcborcid{0000-0003-3160-482X},
C.~Frei$^{50}$\lhcborcid{0000-0001-5501-5611},
D.A.~Friday$^{64,50}$\lhcborcid{0000-0001-9400-3322},
J.~Fu$^{7}$\lhcborcid{0000-0003-3177-2700},
Q.~F{\"u}hring$^{19,g,57}$\lhcborcid{0000-0003-3179-2525},
T.~Fulghesu$^{13}$\lhcborcid{0000-0001-9391-8619},
G.~Galati$^{24}$\lhcborcid{0000-0001-7348-3312},
M.D.~Galati$^{38}$\lhcborcid{0000-0002-8716-4440},
A.~Gallas~Torreira$^{48}$\lhcborcid{0000-0002-2745-7954},
D.~Galli$^{25,k}$\lhcborcid{0000-0003-2375-6030},
S.~Gambetta$^{60}$\lhcborcid{0000-0003-2420-0501},
M.~Gandelman$^{3}$\lhcborcid{0000-0001-8192-8377},
P.~Gandini$^{30}$\lhcborcid{0000-0001-7267-6008},
B. ~Ganie$^{64}$\lhcborcid{0009-0008-7115-3940},
H.~Gao$^{7}$\lhcborcid{0000-0002-6025-6193},
R.~Gao$^{65}$\lhcborcid{0009-0004-1782-7642},
T.Q.~Gao$^{57}$\lhcborcid{0000-0001-7933-0835},
Y.~Gao$^{8}$\lhcborcid{0000-0002-6069-8995},
Y.~Gao$^{6}$\lhcborcid{0000-0003-1484-0943},
Y.~Gao$^{8}$\lhcborcid{0009-0002-5342-4475},
L.M.~Garcia~Martin$^{51}$\lhcborcid{0000-0003-0714-8991},
P.~Garcia~Moreno$^{46}$\lhcborcid{0000-0002-3612-1651},
J.~Garc{\'\i}a~Pardi{\~n}as$^{66}$\lhcborcid{0000-0003-2316-8829},
P. ~Gardner$^{68}$\lhcborcid{0000-0002-8090-563X},
L.~Garrido$^{46}$\lhcborcid{0000-0001-8883-6539},
C.~Gaspar$^{50}$\lhcborcid{0000-0002-8009-1509},
A. ~Gavrikov$^{33}$\lhcborcid{0000-0002-6741-5409},
L.L.~Gerken$^{19}$\lhcborcid{0000-0002-6769-3679},
E.~Gersabeck$^{20}$\lhcborcid{0000-0002-2860-6528},
M.~Gersabeck$^{20}$\lhcborcid{0000-0002-0075-8669},
T.~Gershon$^{58}$\lhcborcid{0000-0002-3183-5065},
S.~Ghizzo$^{29,n}$\lhcborcid{0009-0001-5178-9385},
Z.~Ghorbanimoghaddam$^{56}$\lhcborcid{0000-0002-4410-9505},
F. I.~Giasemis$^{16,f}$\lhcborcid{0000-0003-0622-1069},
V.~Gibson$^{57}$\lhcborcid{0000-0002-6661-1192},
H.K.~Giemza$^{42}$\lhcborcid{0000-0003-2597-8796},
A.L.~Gilman$^{67}$\lhcborcid{0000-0001-5934-7541},
M.~Giovannetti$^{28}$\lhcborcid{0000-0003-2135-9568},
A.~Giovent{\`u}$^{46}$\lhcborcid{0000-0001-5399-326X},
L.~Girardey$^{64,59}$\lhcborcid{0000-0002-8254-7274},
M.A.~Giza$^{41}$\lhcborcid{0000-0002-0805-1561},
F.C.~Glaser$^{14,22}$\lhcborcid{0000-0001-8416-5416},
V.V.~Gligorov$^{16}$\lhcborcid{0000-0002-8189-8267},
C.~G{\"o}bel$^{71}$\lhcborcid{0000-0003-0523-495X},
L. ~Golinka-Bezshyyko$^{87}$\lhcborcid{0000-0002-0613-5374},
E.~Golobardes$^{47}$\lhcborcid{0000-0001-8080-0769},
D.~Golubkov$^{44}$\lhcborcid{0000-0001-6216-1596},
A.~Golutvin$^{63,50}$\lhcborcid{0000-0003-2500-8247},
S.~Gomez~Fernandez$^{46}$\lhcborcid{0000-0002-3064-9834},
W. ~Gomulka$^{40}$\lhcborcid{0009-0003-2873-425X},
I.~Gonçales~Vaz$^{50}$\lhcborcid{0009-0006-4585-2882},
F.~Goncalves~Abrantes$^{65}$\lhcborcid{0000-0002-7318-482X},
M.~Goncerz$^{41}$\lhcborcid{0000-0002-9224-914X},
G.~Gong$^{4,d}$\lhcborcid{0000-0002-7822-3947},
J. A.~Gooding$^{19}$\lhcborcid{0000-0003-3353-9750},
I.V.~Gorelov$^{44}$\lhcborcid{0000-0001-5570-0133},
C.~Gotti$^{31}$\lhcborcid{0000-0003-2501-9608},
E.~Govorkova$^{66}$\lhcborcid{0000-0003-1920-6618},
J.P.~Grabowski$^{30}$\lhcborcid{0000-0001-8461-8382},
L.A.~Granado~Cardoso$^{50}$\lhcborcid{0000-0003-2868-2173},
E.~Graug{\'e}s$^{46}$\lhcborcid{0000-0001-6571-4096},
E.~Graverini$^{51,u}$\lhcborcid{0000-0003-4647-6429},
L.~Grazette$^{58}$\lhcborcid{0000-0001-7907-4261},
G.~Graziani$^{27}$\lhcborcid{0000-0001-8212-846X},
A. T.~Grecu$^{43}$\lhcborcid{0000-0002-7770-1839},
N.A.~Grieser$^{67}$\lhcborcid{0000-0003-0386-4923},
L.~Grillo$^{61}$\lhcborcid{0000-0001-5360-0091},
S.~Gromov$^{44}$\lhcborcid{0000-0002-8967-3644},
C. ~Gu$^{15}$\lhcborcid{0000-0001-5635-6063},
M.~Guarise$^{26}$\lhcborcid{0000-0001-8829-9681},
L. ~Guerry$^{11}$\lhcborcid{0009-0004-8932-4024},
A.-K.~Guseinov$^{51}$\lhcborcid{0000-0002-5115-0581},
E.~Gushchin$^{44}$\lhcborcid{0000-0001-8857-1665},
Y.~Guz$^{6,50}$\lhcborcid{0000-0001-7552-400X},
T.~Gys$^{50}$\lhcborcid{0000-0002-6825-6497},
K.~Habermann$^{18}$\lhcborcid{0009-0002-6342-5965},
T.~Hadavizadeh$^{1}$\lhcborcid{0000-0001-5730-8434},
C.~Hadjivasiliou$^{68}$\lhcborcid{0000-0002-2234-0001},
G.~Haefeli$^{51}$\lhcborcid{0000-0002-9257-839X},
C.~Haen$^{50}$\lhcborcid{0000-0002-4947-2928},
S. ~Haken$^{57}$\lhcborcid{0009-0007-9578-2197},
G. ~Hallett$^{58}$\lhcborcid{0009-0005-1427-6520},
P.M.~Hamilton$^{68}$\lhcborcid{0000-0002-2231-1374},
J.~Hammerich$^{62}$\lhcborcid{0000-0002-5556-1775},
Q.~Han$^{33}$\lhcborcid{0000-0002-7958-2917},
X.~Han$^{22,50}$\lhcborcid{0000-0001-7641-7505},
S.~Hansmann-Menzemer$^{22}$\lhcborcid{0000-0002-3804-8734},
L.~Hao$^{7}$\lhcborcid{0000-0001-8162-4277},
N.~Harnew$^{65}$\lhcborcid{0000-0001-9616-6651},
T. H. ~Harris$^{1}$\lhcborcid{0009-0000-1763-6759},
M.~Hartmann$^{14}$\lhcborcid{0009-0005-8756-0960},
S.~Hashmi$^{40}$\lhcborcid{0000-0003-2714-2706},
J.~He$^{7,e}$\lhcborcid{0000-0002-1465-0077},
N. ~Heatley$^{14}$\lhcborcid{0000-0003-2204-4779},
A. ~Hedes$^{64}$\lhcborcid{0009-0005-2308-4002},
F.~Hemmer$^{50}$\lhcborcid{0000-0001-8177-0856},
C.~Henderson$^{67}$\lhcborcid{0000-0002-6986-9404},
R.~Henderson$^{14}$\lhcborcid{0009-0006-3405-5888},
R.D.L.~Henderson$^{1}$\lhcborcid{0000-0001-6445-4907},
A.M.~Hennequin$^{50}$\lhcborcid{0009-0008-7974-3785},
K.~Hennessy$^{62}$\lhcborcid{0000-0002-1529-8087},
L.~Henry$^{51}$\lhcborcid{0000-0003-3605-832X},
J.~Herd$^{63}$\lhcborcid{0000-0001-7828-3694},
P.~Herrero~Gascon$^{22}$\lhcborcid{0000-0001-6265-8412},
J.~Heuel$^{17}$\lhcborcid{0000-0001-9384-6926},
A. ~Heyn$^{13}$\lhcborcid{0009-0009-2864-9569},
A.~Hicheur$^{3}$\lhcborcid{0000-0002-3712-7318},
G.~Hijano~Mendizabal$^{52}$\lhcborcid{0009-0002-1307-1759},
J.~Horswill$^{64}$\lhcborcid{0000-0002-9199-8616},
R.~Hou$^{8}$\lhcborcid{0000-0002-3139-3332},
Y.~Hou$^{11}$\lhcborcid{0000-0001-6454-278X},
D. C.~Houston$^{61}$\lhcborcid{0009-0003-7753-9565},
N.~Howarth$^{62}$\lhcborcid{0009-0001-7370-061X},
W.~Hu$^{7}$\lhcborcid{0000-0002-2855-0544},
X.~Hu$^{4}$\lhcborcid{0000-0002-5924-2683},
W.~Hulsbergen$^{38}$\lhcborcid{0000-0003-3018-5707},
R.J.~Hunter$^{58}$\lhcborcid{0000-0001-7894-8799},
M.~Hushchyn$^{44}$\lhcborcid{0000-0002-8894-6292},
D.~Hutchcroft$^{62}$\lhcborcid{0000-0002-4174-6509},
M.~Idzik$^{40}$\lhcborcid{0000-0001-6349-0033},
D.~Ilin$^{44}$\lhcborcid{0000-0001-8771-3115},
P.~Ilten$^{67}$\lhcborcid{0000-0001-5534-1732},
A.~Iniukhin$^{44}$\lhcborcid{0000-0002-1940-6276},
A. ~Iohner$^{10}$\lhcborcid{0009-0003-1506-7427},
A.~Ishteev$^{44}$\lhcborcid{0000-0003-1409-1428},
K.~Ivshin$^{44}$\lhcborcid{0000-0001-8403-0706},
H.~Jage$^{17}$\lhcborcid{0000-0002-8096-3792},
S.J.~Jaimes~Elles$^{78,49,50}$\lhcborcid{0000-0003-0182-8638},
S.~Jakobsen$^{50}$\lhcborcid{0000-0002-6564-040X},
T.~Jakoubek$^{79}$\lhcborcid{0000-0001-7038-0369},
E.~Jans$^{38}$\lhcborcid{0000-0002-5438-9176},
B.K.~Jashal$^{49}$\lhcborcid{0000-0002-0025-4663},
A.~Jawahery$^{68}$\lhcborcid{0000-0003-3719-119X},
C. ~Jayaweera$^{55}$\lhcborcid{ 0009-0004-2328-658X},
V.~Jevtic$^{19}$\lhcborcid{0000-0001-6427-4746},
Z. ~Jia$^{16}$\lhcborcid{0000-0002-4774-5961},
E.~Jiang$^{68}$\lhcborcid{0000-0003-1728-8525},
X.~Jiang$^{5,7}$\lhcborcid{0000-0001-8120-3296},
Y.~Jiang$^{7}$\lhcborcid{0000-0002-8964-5109},
Y. J. ~Jiang$^{6}$\lhcborcid{0000-0002-0656-8647},
E.~Jimenez~Moya$^{9}$\lhcborcid{0000-0001-7712-3197},
N. ~Jindal$^{89}$\lhcborcid{0000-0002-2092-3545},
M.~John$^{65}$\lhcborcid{0000-0002-8579-844X},
A. ~John~Rubesh~Rajan$^{23}$\lhcborcid{0000-0002-9850-4965},
D.~Johnson$^{55}$\lhcborcid{0000-0003-3272-6001},
C.R.~Jones$^{57}$\lhcborcid{0000-0003-1699-8816},
S.~Joshi$^{42}$\lhcborcid{0000-0002-5821-1674},
B.~Jost$^{50}$\lhcborcid{0009-0005-4053-1222},
J. ~Juan~Castella$^{57}$\lhcborcid{0009-0009-5577-1308},
N.~Jurik$^{50}$\lhcborcid{0000-0002-6066-7232},
I.~Juszczak$^{41}$\lhcborcid{0000-0002-1285-3911},
K. ~Kalecinska$^{40}$,
D.~Kaminaris$^{51}$\lhcborcid{0000-0002-8912-4653},
S.~Kandybei$^{53}$\lhcborcid{0000-0003-3598-0427},
M. ~Kane$^{60}$\lhcborcid{ 0009-0006-5064-966X},
Y.~Kang$^{4,d}$\lhcborcid{0000-0002-6528-8178},
C.~Kar$^{11}$\lhcborcid{0000-0002-6407-6974},
M.~Karacson$^{50}$\lhcborcid{0009-0006-1867-9674},
A.~Kauniskangas$^{51}$\lhcborcid{0000-0002-4285-8027},
J.W.~Kautz$^{67}$\lhcborcid{0000-0001-8482-5576},
M.K.~Kazanecki$^{41}$\lhcborcid{0009-0009-3480-5724},
F.~Keizer$^{50}$\lhcborcid{0000-0002-1290-6737},
M.~Kenzie$^{57}$\lhcborcid{0000-0001-7910-4109},
T.~Ketel$^{38}$\lhcborcid{0000-0002-9652-1964},
B.~Khanji$^{70}$\lhcborcid{0000-0003-3838-281X},
A.~Kharisova$^{44}$\lhcborcid{0000-0002-5291-9583},
S.~Kholodenko$^{63,50}$\lhcborcid{0000-0002-0260-6570},
G.~Khreich$^{14}$\lhcborcid{0000-0002-6520-8203},
T.~Kirn$^{17}$\lhcborcid{0000-0002-0253-8619},
V.S.~Kirsebom$^{31,p}$\lhcborcid{0009-0005-4421-9025},
S.~Klaver$^{39}$\lhcborcid{0000-0001-7909-1272},
N.~Kleijne$^{35,t}$\lhcborcid{0000-0003-0828-0943},
A.~Kleimenova$^{51}$\lhcborcid{0000-0002-9129-4985},
D. K. ~Klekots$^{87}$\lhcborcid{0000-0002-4251-2958},
K.~Klimaszewski$^{42}$\lhcborcid{0000-0003-0741-5922},
M.R.~Kmiec$^{42}$\lhcborcid{0000-0002-1821-1848},
T. ~Knospe$^{19}$\lhcborcid{ 0009-0003-8343-3767},
R. ~Kolb$^{22}$\lhcborcid{0009-0005-5214-0202},
S.~Koliiev$^{54}$\lhcborcid{0009-0002-3680-1224},
L.~Kolk$^{19}$\lhcborcid{0000-0003-2589-5130},
A.~Konoplyannikov$^{6}$\lhcborcid{0009-0005-2645-8364},
P.~Kopciewicz$^{50}$\lhcborcid{0000-0001-9092-3527},
P.~Koppenburg$^{38}$\lhcborcid{0000-0001-8614-7203},
A. ~Korchin$^{53}$\lhcborcid{0000-0001-7947-170X},
M.~Korolev$^{44}$\lhcborcid{0000-0002-7473-2031},
I.~Kostiuk$^{38}$\lhcborcid{0000-0002-8767-7289},
O.~Kot$^{54}$\lhcborcid{0009-0005-5473-6050},
S.~Kotriakhova$^{}$\lhcborcid{0000-0002-1495-0053},
E. ~Kowalczyk$^{68}$\lhcborcid{0009-0006-0206-2784},
A.~Kozachuk$^{44}$\lhcborcid{0000-0001-6805-0395},
P.~Kravchenko$^{44}$\lhcborcid{0000-0002-4036-2060},
L.~Kravchuk$^{44}$\lhcborcid{0000-0001-8631-4200},
O. ~Kravcov$^{82}$\lhcborcid{0000-0001-7148-3335},
M.~Kreps$^{58}$\lhcborcid{0000-0002-6133-486X},
P.~Krokovny$^{44}$\lhcborcid{0000-0002-1236-4667},
W.~Krupa$^{70}$\lhcborcid{0000-0002-7947-465X},
W.~Krzemien$^{42}$\lhcborcid{0000-0002-9546-358X},
O.~Kshyvanskyi$^{54}$\lhcborcid{0009-0003-6637-841X},
S.~Kubis$^{85}$\lhcborcid{0000-0001-8774-8270},
M.~Kucharczyk$^{41}$\lhcborcid{0000-0003-4688-0050},
V.~Kudryavtsev$^{44}$\lhcborcid{0009-0000-2192-995X},
E.~Kulikova$^{44}$\lhcborcid{0009-0002-8059-5325},
A.~Kupsc$^{86}$\lhcborcid{0000-0003-4937-2270},
V.~Kushnir$^{53}$\lhcborcid{0000-0003-2907-1323},
B.~Kutsenko$^{13}$\lhcborcid{0000-0002-8366-1167},
J.~Kvapil$^{69}$\lhcborcid{0000-0002-0298-9073},
I. ~Kyryllin$^{53}$\lhcborcid{0000-0003-3625-7521},
D.~Lacarrere$^{50}$\lhcborcid{0009-0005-6974-140X},
P. ~Laguarta~Gonzalez$^{46}$\lhcborcid{0009-0005-3844-0778},
A.~Lai$^{32}$\lhcborcid{0000-0003-1633-0496},
A.~Lampis$^{32}$\lhcborcid{0000-0002-5443-4870},
D.~Lancierini$^{63}$\lhcborcid{0000-0003-1587-4555},
C.~Landesa~Gomez$^{48}$\lhcborcid{0000-0001-5241-8642},
J.J.~Lane$^{1}$\lhcborcid{0000-0002-5816-9488},
G.~Lanfranchi$^{28}$\lhcborcid{0000-0002-9467-8001},
C.~Langenbruch$^{22}$\lhcborcid{0000-0002-3454-7261},
J.~Langer$^{19}$\lhcborcid{0000-0002-0322-5550},
T.~Latham$^{58}$\lhcborcid{0000-0002-7195-8537},
F.~Lazzari$^{35,u,50}$\lhcborcid{0000-0002-3151-3453},
C.~Lazzeroni$^{55}$\lhcborcid{0000-0003-4074-4787},
R.~Le~Gac$^{13}$\lhcborcid{0000-0002-7551-6971},
H. ~Lee$^{62}$\lhcborcid{0009-0003-3006-2149},
R.~Lef{\`e}vre$^{11}$\lhcborcid{0000-0002-6917-6210},
A.~Leflat$^{44}$\lhcborcid{0000-0001-9619-6666},
S.~Legotin$^{44}$\lhcborcid{0000-0003-3192-6175},
M.~Lehuraux$^{58}$\lhcborcid{0000-0001-7600-7039},
E.~Lemos~Cid$^{50}$\lhcborcid{0000-0003-3001-6268},
O.~Leroy$^{13}$\lhcborcid{0000-0002-2589-240X},
T.~Lesiak$^{41}$\lhcborcid{0000-0002-3966-2998},
E. D.~Lesser$^{50}$\lhcborcid{0000-0001-8367-8703},
B.~Leverington$^{22}$\lhcborcid{0000-0001-6640-7274},
A.~Li$^{4,d}$\lhcborcid{0000-0001-5012-6013},
C. ~Li$^{4,d}$\lhcborcid{0009-0002-3366-2871},
C. ~Li$^{13}$\lhcborcid{0000-0002-3554-5479},
H.~Li$^{74}$\lhcborcid{0000-0002-2366-9554},
J.~Li$^{8}$\lhcborcid{0009-0003-8145-0643},
K.~Li$^{77}$\lhcborcid{0000-0002-2243-8412},
L.~Li$^{64}$\lhcborcid{0000-0003-4625-6880},
M.~Li$^{8}$\lhcborcid{0009-0002-3024-1545},
P.~Li$^{7}$\lhcborcid{0000-0003-2740-9765},
P.-R.~Li$^{75}$\lhcborcid{0000-0002-1603-3646},
Q. ~Li$^{5,7}$\lhcborcid{0009-0004-1932-8580},
T.~Li$^{73}$\lhcborcid{0000-0002-5241-2555},
T.~Li$^{74}$\lhcborcid{0000-0002-5723-0961},
Y.~Li$^{8}$\lhcborcid{0009-0004-0130-6121},
Y.~Li$^{5}$\lhcborcid{0000-0003-2043-4669},
Y. ~Li$^{4}$\lhcborcid{0009-0007-6670-7016},
Z.~Lian$^{4,d}$\lhcborcid{0000-0003-4602-6946},
Q. ~Liang$^{8}$,
X.~Liang$^{70}$\lhcborcid{0000-0002-5277-9103},
Z. ~Liang$^{32}$\lhcborcid{0000-0001-6027-6883},
S.~Libralon$^{49}$\lhcborcid{0009-0002-5841-9624},
A. L. ~Lightbody$^{12}$\lhcborcid{0009-0008-9092-582X},
C.~Lin$^{7}$\lhcborcid{0000-0001-7587-3365},
T.~Lin$^{59}$\lhcborcid{0000-0001-6052-8243},
R.~Lindner$^{50}$\lhcborcid{0000-0002-5541-6500},
H. ~Linton$^{63}$\lhcborcid{0009-0000-3693-1972},
R.~Litvinov$^{32}$\lhcborcid{0000-0002-4234-435X},
D.~Liu$^{8}$\lhcborcid{0009-0002-8107-5452},
F. L. ~Liu$^{1}$\lhcborcid{0009-0002-2387-8150},
G.~Liu$^{74}$\lhcborcid{0000-0001-5961-6588},
K.~Liu$^{75}$\lhcborcid{0000-0003-4529-3356},
S.~Liu$^{5}$\lhcborcid{0000-0002-6919-227X},
W. ~Liu$^{8}$\lhcborcid{0009-0005-0734-2753},
Y.~Liu$^{60}$\lhcborcid{0000-0003-3257-9240},
Y.~Liu$^{75}$\lhcborcid{0009-0002-0885-5145},
Y. L. ~Liu$^{63}$\lhcborcid{0000-0001-9617-6067},
G.~Loachamin~Ordonez$^{71}$\lhcborcid{0009-0001-3549-3939},
I. ~Lobo$^{1}$\lhcborcid{0009-0003-3915-4146},
A.~Lobo~Salvia$^{46}$\lhcborcid{0000-0002-2375-9509},
A.~Loi$^{32}$\lhcborcid{0000-0003-4176-1503},
T.~Long$^{57}$\lhcborcid{0000-0001-7292-848X},
F. C. L.~Lopes$^{2,a}$\lhcborcid{0009-0006-1335-3595},
J.H.~Lopes$^{3}$\lhcborcid{0000-0003-1168-9547},
A.~Lopez~Huertas$^{46}$\lhcborcid{0000-0002-6323-5582},
C. ~Lopez~Iribarnegaray$^{48}$\lhcborcid{0009-0004-3953-6694},
S.~L{\'o}pez~Soli{\~n}o$^{48}$\lhcborcid{0000-0001-9892-5113},
Q.~Lu$^{15}$\lhcborcid{0000-0002-6598-1941},
C.~Lucarelli$^{50}$\lhcborcid{0000-0002-8196-1828},
D.~Lucchesi$^{33,r}$\lhcborcid{0000-0003-4937-7637},
M.~Lucio~Martinez$^{49}$\lhcborcid{0000-0001-6823-2607},
Y.~Luo$^{6}$\lhcborcid{0009-0001-8755-2937},
A.~Lupato$^{33,j}$\lhcborcid{0000-0003-0312-3914},
E.~Luppi$^{26,m}$\lhcborcid{0000-0002-1072-5633},
K.~Lynch$^{23}$\lhcborcid{0000-0002-7053-4951},
X.-R.~Lyu$^{7}$\lhcborcid{0000-0001-5689-9578},
G. M. ~Ma$^{4,d}$\lhcborcid{0000-0001-8838-5205},
H. ~Ma$^{73}$\lhcborcid{0009-0001-0655-6494},
S.~Maccolini$^{19}$\lhcborcid{0000-0002-9571-7535},
F.~Machefert$^{14}$\lhcborcid{0000-0002-4644-5916},
F.~Maciuc$^{43}$\lhcborcid{0000-0001-6651-9436},
B. ~Mack$^{70}$\lhcborcid{0000-0001-8323-6454},
I.~Mackay$^{65}$\lhcborcid{0000-0003-0171-7890},
L. M. ~Mackey$^{70}$\lhcborcid{0000-0002-8285-3589},
L.R.~Madhan~Mohan$^{57}$\lhcborcid{0000-0002-9390-8821},
M. J. ~Madurai$^{55}$\lhcborcid{0000-0002-6503-0759},
D.~Magdalinski$^{38}$\lhcborcid{0000-0001-6267-7314},
D.~Maisuzenko$^{44}$\lhcborcid{0000-0001-5704-3499},
J.J.~Malczewski$^{41}$\lhcborcid{0000-0003-2744-3656},
S.~Malde$^{65}$\lhcborcid{0000-0002-8179-0707},
L.~Malentacca$^{50}$\lhcborcid{0000-0001-6717-2980},
A.~Malinin$^{44}$\lhcborcid{0000-0002-3731-9977},
T.~Maltsev$^{44}$\lhcborcid{0000-0002-2120-5633},
G.~Manca$^{32,l}$\lhcborcid{0000-0003-1960-4413},
G.~Mancinelli$^{13}$\lhcborcid{0000-0003-1144-3678},
C.~Mancuso$^{14}$\lhcborcid{0000-0002-2490-435X},
R.~Manera~Escalero$^{46}$\lhcborcid{0000-0003-4981-6847},
F. M. ~Manganella$^{37}$\lhcborcid{0009-0003-1124-0974},
D.~Manuzzi$^{25}$\lhcborcid{0000-0002-9915-6587},
D.~Marangotto$^{30,o}$\lhcborcid{0000-0001-9099-4878},
J.F.~Marchand$^{10}$\lhcborcid{0000-0002-4111-0797},
R.~Marchevski$^{51}$\lhcborcid{0000-0003-3410-0918},
U.~Marconi$^{25}$\lhcborcid{0000-0002-5055-7224},
E.~Mariani$^{16}$\lhcborcid{0009-0002-3683-2709},
S.~Mariani$^{50}$\lhcborcid{0000-0002-7298-3101},
C.~Marin~Benito$^{46}$\lhcborcid{0000-0003-0529-6982},
J.~Marks$^{22}$\lhcborcid{0000-0002-2867-722X},
A.M.~Marshall$^{56}$\lhcborcid{0000-0002-9863-4954},
L. ~Martel$^{65}$\lhcborcid{0000-0001-8562-0038},
G.~Martelli$^{34}$\lhcborcid{0000-0002-6150-3168},
G.~Martellotti$^{36}$\lhcborcid{0000-0002-8663-9037},
L.~Martinazzoli$^{50}$\lhcborcid{0000-0002-8996-795X},
M.~Martinelli$^{31,p}$\lhcborcid{0000-0003-4792-9178},
D. ~Martinez~Gomez$^{83}$\lhcborcid{0009-0001-2684-9139},
D.~Martinez~Santos$^{45}$\lhcborcid{0000-0002-6438-4483},
F.~Martinez~Vidal$^{49}$\lhcborcid{0000-0001-6841-6035},
A. ~Martorell~i~Granollers$^{47}$\lhcborcid{0009-0005-6982-9006},
A.~Massafferri$^{2}$\lhcborcid{0000-0002-3264-3401},
R.~Matev$^{50}$\lhcborcid{0000-0001-8713-6119},
A.~Mathad$^{50}$\lhcborcid{0000-0002-9428-4715},
V.~Matiunin$^{44}$\lhcborcid{0000-0003-4665-5451},
C.~Matteuzzi$^{70}$\lhcborcid{0000-0002-4047-4521},
K.R.~Mattioli$^{15}$\lhcborcid{0000-0003-2222-7727},
A.~Mauri$^{63}$\lhcborcid{0000-0003-1664-8963},
E.~Maurice$^{15}$\lhcborcid{0000-0002-7366-4364},
J.~Mauricio$^{46}$\lhcborcid{0000-0002-9331-1363},
P.~Mayencourt$^{51}$\lhcborcid{0000-0002-8210-1256},
J.~Mazorra~de~Cos$^{49}$\lhcborcid{0000-0003-0525-2736},
M.~Mazurek$^{42}$\lhcborcid{0000-0002-3687-9630},
M.~McCann$^{63}$\lhcborcid{0000-0002-3038-7301},
N.T.~McHugh$^{61}$\lhcborcid{0000-0002-5477-3995},
A.~McNab$^{64}$\lhcborcid{0000-0001-5023-2086},
R.~McNulty$^{23}$\lhcborcid{0000-0001-7144-0175},
B.~Meadows$^{67}$\lhcborcid{0000-0002-1947-8034},
G.~Meier$^{19}$\lhcborcid{0000-0002-4266-1726},
D.~Melnychuk$^{42}$\lhcborcid{0000-0003-1667-7115},
D.~Mendoza~Granada$^{16}$\lhcborcid{0000-0002-6459-5408},
P. ~Menendez~Valdes~Perez$^{48}$\lhcborcid{0009-0003-0406-8141},
F. M. ~Meng$^{4,d}$\lhcborcid{0009-0004-1533-6014},
M.~Merk$^{38,84}$\lhcborcid{0000-0003-0818-4695},
A.~Merli$^{51,30}$\lhcborcid{0000-0002-0374-5310},
L.~Meyer~Garcia$^{68}$\lhcborcid{0000-0002-2622-8551},
D.~Miao$^{5,7}$\lhcborcid{0000-0003-4232-5615},
H.~Miao$^{7}$\lhcborcid{0000-0002-1936-5400},
M.~Mikhasenko$^{80}$\lhcborcid{0000-0002-6969-2063},
D.A.~Milanes$^{78,y}$\lhcborcid{0000-0001-7450-1121},
A.~Minotti$^{31,p}$\lhcborcid{0000-0002-0091-5177},
E.~Minucci$^{28}$\lhcborcid{0000-0002-3972-6824},
T.~Miralles$^{11}$\lhcborcid{0000-0002-4018-1454},
B.~Mitreska$^{64}$\lhcborcid{0000-0002-1697-4999},
D.S.~Mitzel$^{19}$\lhcborcid{0000-0003-3650-2689},
R. ~Mocanu$^{43}$\lhcborcid{0009-0005-5391-7255},
A.~Modak$^{59}$\lhcborcid{0000-0003-1198-1441},
L.~Moeser$^{19}$\lhcborcid{0009-0007-2494-8241},
R.D.~Moise$^{17}$\lhcborcid{0000-0002-5662-8804},
E. F.~Molina~Cardenas$^{88}$\lhcborcid{0009-0002-0674-5305},
T.~Momb{\"a}cher$^{67}$\lhcborcid{0000-0002-5612-979X},
M.~Monk$^{57}$\lhcborcid{0000-0003-0484-0157},
T.~Monnard$^{51}$\lhcborcid{0009-0005-7171-7775},
S.~Monteil$^{11}$\lhcborcid{0000-0001-5015-3353},
A.~Morcillo~Gomez$^{48}$\lhcborcid{0000-0001-9165-7080},
G.~Morello$^{28}$\lhcborcid{0000-0002-6180-3697},
M.J.~Morello$^{35,t}$\lhcborcid{0000-0003-4190-1078},
M.P.~Morgenthaler$^{22}$\lhcborcid{0000-0002-7699-5724},
A. ~Moro$^{31,p}$\lhcborcid{0009-0007-8141-2486},
J.~Moron$^{40}$\lhcborcid{0000-0002-1857-1675},
W. ~Morren$^{38}$\lhcborcid{0009-0004-1863-9344},
A.B.~Morris$^{50}$\lhcborcid{0000-0002-0832-9199},
A.G.~Morris$^{13}$\lhcborcid{0000-0001-6644-9888},
R.~Mountain$^{70}$\lhcborcid{0000-0003-1908-4219},
Z. M. ~Mu$^{6}$\lhcborcid{0000-0001-9291-2231},
E.~Muhammad$^{58}$\lhcborcid{0000-0001-7413-5862},
F.~Muheim$^{60}$\lhcborcid{0000-0002-1131-8909},
M.~Mulder$^{83}$\lhcborcid{0000-0001-6867-8166},
K.~M{\"u}ller$^{52}$\lhcborcid{0000-0002-5105-1305},
F.~Mu{\~n}oz-Rojas$^{9}$\lhcborcid{0000-0002-4978-602X},
R.~Murta$^{63}$\lhcborcid{0000-0002-6915-8370},
V. ~Mytrochenko$^{53}$\lhcborcid{ 0000-0002-3002-7402},
P.~Naik$^{62}$\lhcborcid{0000-0001-6977-2971},
T.~Nakada$^{51}$\lhcborcid{0009-0000-6210-6861},
R.~Nandakumar$^{59}$\lhcborcid{0000-0002-6813-6794},
T.~Nanut$^{50}$\lhcborcid{0000-0002-5728-9867},
G. ~Napoletano$^{51}$\lhcborcid{0009-0008-9225-8653},
I.~Nasteva$^{3}$\lhcborcid{0000-0001-7115-7214},
M.~Needham$^{60}$\lhcborcid{0000-0002-8297-6714},
E. ~Nekrasova$^{44}$\lhcborcid{0009-0009-5725-2405},
N.~Neri$^{30,o}$\lhcborcid{0000-0002-6106-3756},
S.~Neubert$^{18}$\lhcborcid{0000-0002-0706-1944},
N.~Neufeld$^{50}$\lhcborcid{0000-0003-2298-0102},
P.~Neustroev$^{44}$,
J.~Nicolini$^{50}$\lhcborcid{0000-0001-9034-3637},
D.~Nicotra$^{84}$\lhcborcid{0000-0001-7513-3033},
E.M.~Niel$^{15}$\lhcborcid{0000-0002-6587-4695},
N.~Nikitin$^{44}$\lhcborcid{0000-0003-0215-1091},
L. ~Nisi$^{19}$\lhcborcid{0009-0006-8445-8968},
Q.~Niu$^{75}$\lhcborcid{0009-0004-3290-2444},
P.~Nogarolli$^{3}$\lhcborcid{0009-0001-4635-1055},
P.~Nogga$^{18}$\lhcborcid{0009-0006-2269-4666},
C.~Normand$^{56}$\lhcborcid{0000-0001-5055-7710},
J.~Novoa~Fernandez$^{48}$\lhcborcid{0000-0002-1819-1381},
G.~Nowak$^{67}$\lhcborcid{0000-0003-4864-7164},
C.~Nunez$^{88}$\lhcborcid{0000-0002-2521-9346},
H. N. ~Nur$^{61}$\lhcborcid{0000-0002-7822-523X},
A.~Oblakowska-Mucha$^{40}$\lhcborcid{0000-0003-1328-0534},
V.~Obraztsov$^{44}$\lhcborcid{0000-0002-0994-3641},
T.~Oeser$^{17}$\lhcborcid{0000-0001-7792-4082},
A.~Okhotnikov$^{44}$,
O.~Okhrimenko$^{54}$\lhcborcid{0000-0002-0657-6962},
R.~Oldeman$^{32,l}$\lhcborcid{0000-0001-6902-0710},
F.~Oliva$^{60,50}$\lhcborcid{0000-0001-7025-3407},
E. ~Olivart~Pino$^{46}$\lhcborcid{0009-0001-9398-8614},
M.~Olocco$^{19}$\lhcborcid{0000-0002-6968-1217},
R.H.~O'Neil$^{50}$\lhcborcid{0000-0002-9797-8464},
J.S.~Ordonez~Soto$^{11}$\lhcborcid{0009-0009-0613-4871},
D.~Osthues$^{19}$\lhcborcid{0009-0004-8234-513X},
J.M.~Otalora~Goicochea$^{3}$\lhcborcid{0000-0002-9584-8500},
P.~Owen$^{52}$\lhcborcid{0000-0002-4161-9147},
A.~Oyanguren$^{49}$\lhcborcid{0000-0002-8240-7300},
O.~Ozcelik$^{50}$\lhcborcid{0000-0003-3227-9248},
F.~Paciolla$^{35,w}$\lhcborcid{0000-0002-6001-600X},
A. ~Padee$^{42}$\lhcborcid{0000-0002-5017-7168},
K.O.~Padeken$^{18}$\lhcborcid{0000-0001-7251-9125},
B.~Pagare$^{48}$\lhcborcid{0000-0003-3184-1622},
T.~Pajero$^{50}$\lhcborcid{0000-0001-9630-2000},
A.~Palano$^{24}$\lhcborcid{0000-0002-6095-9593},
L. ~Palini$^{30}$\lhcborcid{0009-0004-4010-2172},
M.~Palutan$^{28}$\lhcborcid{0000-0001-7052-1360},
C. ~Pan$^{76}$\lhcborcid{0009-0009-9985-9950},
X. ~Pan$^{4,d}$\lhcborcid{0000-0002-7439-6621},
S.~Panebianco$^{12}$\lhcborcid{0000-0002-0343-2082},
S.~Paniskaki$^{50,33}$\lhcborcid{0009-0004-4947-954X},
G.~Panshin$^{5}$\lhcborcid{0000-0001-9163-2051},
L.~Paolucci$^{64}$\lhcborcid{0000-0003-0465-2893},
A.~Papanestis$^{59}$\lhcborcid{0000-0002-5405-2901},
M.~Pappagallo$^{24,i}$\lhcborcid{0000-0001-7601-5602},
L.L.~Pappalardo$^{26}$\lhcborcid{0000-0002-0876-3163},
C.~Pappenheimer$^{67}$\lhcborcid{0000-0003-0738-3668},
C.~Parkes$^{64}$\lhcborcid{0000-0003-4174-1334},
D. ~Parmar$^{80}$\lhcborcid{0009-0004-8530-7630},
G.~Passaleva$^{27}$\lhcborcid{0000-0002-8077-8378},
D.~Passaro$^{35,t,50}$\lhcborcid{0000-0002-8601-2197},
A.~Pastore$^{24}$\lhcborcid{0000-0002-5024-3495},
M.~Patel$^{63}$\lhcborcid{0000-0003-3871-5602},
J.~Patoc$^{65}$\lhcborcid{0009-0000-1201-4918},
C.~Patrignani$^{25,k}$\lhcborcid{0000-0002-5882-1747},
A. ~Paul$^{70}$\lhcborcid{0009-0006-7202-0811},
C.J.~Pawley$^{84}$\lhcborcid{0000-0001-9112-3724},
A.~Pellegrino$^{38}$\lhcborcid{0000-0002-7884-345X},
J. ~Peng$^{5,7}$\lhcborcid{0009-0005-4236-4667},
X. ~Peng$^{75}$,
M.~Pepe~Altarelli$^{28}$\lhcborcid{0000-0002-1642-4030},
S.~Perazzini$^{25}$\lhcborcid{0000-0002-1862-7122},
D.~Pereima$^{44}$\lhcborcid{0000-0002-7008-8082},
H. ~Pereira~Da~Costa$^{69}$\lhcborcid{0000-0002-3863-352X},
M. ~Pereira~Martinez$^{48}$\lhcborcid{0009-0006-8577-9560},
A.~Pereiro~Castro$^{48}$\lhcborcid{0000-0001-9721-3325},
C. ~Perez$^{47}$\lhcborcid{0000-0002-6861-2674},
P.~Perret$^{11}$\lhcborcid{0000-0002-5732-4343},
A. ~Perrevoort$^{83}$\lhcborcid{0000-0001-6343-447X},
A.~Perro$^{50,13}$\lhcborcid{0000-0002-1996-0496},
M.J.~Peters$^{67}$\lhcborcid{0009-0008-9089-1287},
K.~Petridis$^{56}$\lhcborcid{0000-0001-7871-5119},
A.~Petrolini$^{29,n}$\lhcborcid{0000-0003-0222-7594},
S. ~Pezzulo$^{29,n}$\lhcborcid{0009-0004-4119-4881},
J. P. ~Pfaller$^{67}$\lhcborcid{0009-0009-8578-3078},
H.~Pham$^{70}$\lhcborcid{0000-0003-2995-1953},
L.~Pica$^{35,t}$\lhcborcid{0000-0001-9837-6556},
M.~Piccini$^{34}$\lhcborcid{0000-0001-8659-4409},
L. ~Piccolo$^{32}$\lhcborcid{0000-0003-1896-2892},
B.~Pietrzyk$^{10}$\lhcborcid{0000-0003-1836-7233},
G.~Pietrzyk$^{14}$\lhcborcid{0000-0001-9622-820X},
R. N.~Pilato$^{62}$\lhcborcid{0000-0002-4325-7530},
D.~Pinci$^{36}$\lhcborcid{0000-0002-7224-9708},
F.~Pisani$^{50}$\lhcborcid{0000-0002-7763-252X},
M.~Pizzichemi$^{31,p,50}$\lhcborcid{0000-0001-5189-230X},
V. M.~Placinta$^{43}$\lhcborcid{0000-0003-4465-2441},
M.~Plo~Casasus$^{48}$\lhcborcid{0000-0002-2289-918X},
T.~Poeschl$^{50}$\lhcborcid{0000-0003-3754-7221},
F.~Polci$^{16}$\lhcborcid{0000-0001-8058-0436},
M.~Poli~Lener$^{28}$\lhcborcid{0000-0001-7867-1232},
A.~Poluektov$^{13}$\lhcborcid{0000-0003-2222-9925},
N.~Polukhina$^{44}$\lhcborcid{0000-0001-5942-1772},
I.~Polyakov$^{64}$\lhcborcid{0000-0002-6855-7783},
E.~Polycarpo$^{3}$\lhcborcid{0000-0002-4298-5309},
S.~Ponce$^{50}$\lhcborcid{0000-0002-1476-7056},
D.~Popov$^{7,50}$\lhcborcid{0000-0002-8293-2922},
K.~Popp$^{19}$\lhcborcid{0009-0002-6372-2767},
S.~Poslavskii$^{44}$\lhcborcid{0000-0003-3236-1452},
K.~Prasanth$^{60}$\lhcborcid{0000-0001-9923-0938},
C.~Prouve$^{45}$\lhcborcid{0000-0003-2000-6306},
D.~Provenzano$^{32,l,50}$\lhcborcid{0009-0005-9992-9761},
V.~Pugatch$^{54}$\lhcborcid{0000-0002-5204-9821},
A. ~Puicercus~Gomez$^{50}$\lhcborcid{0009-0005-9982-6383},
G.~Punzi$^{35,u}$\lhcborcid{0000-0002-8346-9052},
J.R.~Pybus$^{69}$\lhcborcid{0000-0001-8951-2317},
Q. Q. ~Qian$^{6}$\lhcborcid{0000-0001-6453-4691},
W.~Qian$^{7}$\lhcborcid{0000-0003-3932-7556},
N.~Qin$^{4,d}$\lhcborcid{0000-0001-8453-658X},
R.~Quagliani$^{50}$\lhcborcid{0000-0002-3632-2453},
R.I.~Rabadan~Trejo$^{58}$\lhcborcid{0000-0002-9787-3910},
R. ~Racz$^{82}$\lhcborcid{0009-0003-3834-8184},
J.H.~Rademacker$^{56}$\lhcborcid{0000-0003-2599-7209},
M.~Rama$^{35}$\lhcborcid{0000-0003-3002-4719},
M. ~Ram\'{i}rez~Garc\'{i}a$^{88}$\lhcborcid{0000-0001-7956-763X},
V.~Ramos~De~Oliveira$^{71}$\lhcborcid{0000-0003-3049-7866},
M.~Ramos~Pernas$^{58}$\lhcborcid{0000-0003-1600-9432},
M.S.~Rangel$^{3}$\lhcborcid{0000-0002-8690-5198},
F.~Ratnikov$^{44}$\lhcborcid{0000-0003-0762-5583},
G.~Raven$^{39}$\lhcborcid{0000-0002-2897-5323},
M.~Rebollo~De~Miguel$^{49}$\lhcborcid{0000-0002-4522-4863},
F.~Redi$^{30,j}$\lhcborcid{0000-0001-9728-8984},
J.~Reich$^{56}$\lhcborcid{0000-0002-2657-4040},
F.~Reiss$^{20}$\lhcborcid{0000-0002-8395-7654},
Z.~Ren$^{7}$\lhcborcid{0000-0001-9974-9350},
P.K.~Resmi$^{65}$\lhcborcid{0000-0001-9025-2225},
M. ~Ribalda~Galvez$^{46}$\lhcborcid{0009-0006-0309-7639},
R.~Ribatti$^{51}$\lhcborcid{0000-0003-1778-1213},
G.~Ricart$^{12}$\lhcborcid{0000-0002-9292-2066},
D.~Riccardi$^{35,t}$\lhcborcid{0009-0009-8397-572X},
S.~Ricciardi$^{59}$\lhcborcid{0000-0002-4254-3658},
K.~Richardson$^{66}$\lhcborcid{0000-0002-6847-2835},
M.~Richardson-Slipper$^{57}$\lhcborcid{0000-0002-2752-001X},
F. ~Riehn$^{19}$\lhcborcid{ 0000-0001-8434-7500},
K.~Rinnert$^{62}$\lhcborcid{0000-0001-9802-1122},
P.~Robbe$^{14,50}$\lhcborcid{0000-0002-0656-9033},
G.~Robertson$^{61}$\lhcborcid{0000-0002-7026-1383},
E.~Rodrigues$^{62}$\lhcborcid{0000-0003-2846-7625},
A.~Rodriguez~Alvarez$^{46}$\lhcborcid{0009-0006-1758-936X},
E.~Rodriguez~Fernandez$^{48}$\lhcborcid{0000-0002-3040-065X},
J.A.~Rodriguez~Lopez$^{78}$\lhcborcid{0000-0003-1895-9319},
E.~Rodriguez~Rodriguez$^{50}$\lhcborcid{0000-0002-7973-8061},
J.~Roensch$^{19}$\lhcborcid{0009-0001-7628-6063},
A.~Rogachev$^{44}$\lhcborcid{0000-0002-7548-6530},
A.~Rogovskiy$^{59}$\lhcborcid{0000-0002-1034-1058},
D.L.~Rolf$^{19}$\lhcborcid{0000-0001-7908-7214},
P.~Roloff$^{50}$\lhcborcid{0000-0001-7378-4350},
V.~Romanovskiy$^{67}$\lhcborcid{0000-0003-0939-4272},
A.~Romero~Vidal$^{48}$\lhcborcid{0000-0002-8830-1486},
G.~Romolini$^{26,50}$\lhcborcid{0000-0002-0118-4214},
F.~Ronchetti$^{51}$\lhcborcid{0000-0003-3438-9774},
T.~Rong$^{6}$\lhcborcid{0000-0002-5479-9212},
M.~Rotondo$^{28}$\lhcborcid{0000-0001-5704-6163},
S. R. ~Roy$^{22}$\lhcborcid{0000-0002-3999-6795},
M.S.~Rudolph$^{70}$\lhcborcid{0000-0002-0050-575X},
M.~Ruiz~Diaz$^{22}$\lhcborcid{0000-0001-6367-6815},
R.A.~Ruiz~Fernandez$^{48}$\lhcborcid{0000-0002-5727-4454},
J.~Ruiz~Vidal$^{84}$\lhcborcid{0000-0001-8362-7164},
J. J.~Saavedra-Arias$^{9}$\lhcborcid{0000-0002-2510-8929},
J.J.~Saborido~Silva$^{48}$\lhcborcid{0000-0002-6270-130X},
S. E. R.~Sacha~Emile~R.$^{50}$\lhcborcid{0000-0002-1432-2858},
N.~Sagidova$^{44}$\lhcborcid{0000-0002-2640-3794},
D.~Sahoo$^{81}$\lhcborcid{0000-0002-5600-9413},
N.~Sahoo$^{55}$\lhcborcid{0000-0001-9539-8370},
B.~Saitta$^{32}$\lhcborcid{0000-0003-3491-0232},
M.~Salomoni$^{31,50,p}$\lhcborcid{0009-0007-9229-653X},
I.~Sanderswood$^{49}$\lhcborcid{0000-0001-7731-6757},
R.~Santacesaria$^{36}$\lhcborcid{0000-0003-3826-0329},
C.~Santamarina~Rios$^{48}$\lhcborcid{0000-0002-9810-1816},
M.~Santimaria$^{28}$\lhcborcid{0000-0002-8776-6759},
L.~Santoro~$^{2}$\lhcborcid{0000-0002-2146-2648},
E.~Santovetti$^{37}$\lhcborcid{0000-0002-5605-1662},
A.~Saputi$^{26,50}$\lhcborcid{0000-0001-6067-7863},
D.~Saranin$^{44}$\lhcborcid{0000-0002-9617-9986},
A.~Sarnatskiy$^{83}$\lhcborcid{0009-0007-2159-3633},
G.~Sarpis$^{50}$\lhcborcid{0000-0003-1711-2044},
M.~Sarpis$^{82}$\lhcborcid{0000-0002-6402-1674},
C.~Satriano$^{36}$\lhcborcid{0000-0002-4976-0460},
A.~Satta$^{37}$\lhcborcid{0000-0003-2462-913X},
M.~Saur$^{75}$\lhcborcid{0000-0001-8752-4293},
D.~Savrina$^{44}$\lhcborcid{0000-0001-8372-6031},
H.~Sazak$^{17}$\lhcborcid{0000-0003-2689-1123},
F.~Sborzacchi$^{50,28}$\lhcborcid{0009-0004-7916-2682},
A.~Scarabotto$^{19}$\lhcborcid{0000-0003-2290-9672},
S.~Schael$^{17}$\lhcborcid{0000-0003-4013-3468},
S.~Scherl$^{62}$\lhcborcid{0000-0003-0528-2724},
M.~Schiller$^{22}$\lhcborcid{0000-0001-8750-863X},
H.~Schindler$^{50}$\lhcborcid{0000-0002-1468-0479},
M.~Schmelling$^{21}$\lhcborcid{0000-0003-3305-0576},
B.~Schmidt$^{50}$\lhcborcid{0000-0002-8400-1566},
N.~Schmidt$^{69}$\lhcborcid{0000-0002-5795-4871},
S.~Schmitt$^{66}$\lhcborcid{0000-0002-6394-1081},
H.~Schmitz$^{18}$,
O.~Schneider$^{51}$\lhcborcid{0000-0002-6014-7552},
A.~Schopper$^{63}$\lhcborcid{0000-0002-8581-3312},
N.~Schulte$^{19}$\lhcborcid{0000-0003-0166-2105},
M.H.~Schune$^{14}$\lhcborcid{0000-0002-3648-0830},
G.~Schwering$^{17}$\lhcborcid{0000-0003-1731-7939},
B.~Sciascia$^{28}$\lhcborcid{0000-0003-0670-006X},
A.~Sciuccati$^{50}$\lhcborcid{0000-0002-8568-1487},
G. ~Scriven$^{84}$\lhcborcid{0009-0004-9997-1647},
I.~Segal$^{80}$\lhcborcid{0000-0001-8605-3020},
S.~Sellam$^{48}$\lhcborcid{0000-0003-0383-1451},
A.~Semennikov$^{44}$\lhcborcid{0000-0003-1130-2197},
T.~Senger$^{52}$\lhcborcid{0009-0006-2212-6431},
M.~Senghi~Soares$^{39}$\lhcborcid{0000-0001-9676-6059},
A.~Sergi$^{29,n}$\lhcborcid{0000-0001-9495-6115},
N.~Serra$^{52}$\lhcborcid{0000-0002-5033-0580},
L.~Sestini$^{27}$\lhcborcid{0000-0002-1127-5144},
A.~Seuthe$^{19}$\lhcborcid{0000-0002-0736-3061},
B. ~Sevilla~Sanjuan$^{47}$\lhcborcid{0009-0002-5108-4112},
Y.~Shang$^{6}$\lhcborcid{0000-0001-7987-7558},
D.M.~Shangase$^{88}$\lhcborcid{0000-0002-0287-6124},
M.~Shapkin$^{44}$\lhcborcid{0000-0002-4098-9592},
R. S. ~Sharma$^{70}$\lhcborcid{0000-0003-1331-1791},
I.~Shchemerov$^{44}$\lhcborcid{0000-0001-9193-8106},
L.~Shchutska$^{51}$\lhcborcid{0000-0003-0700-5448},
T.~Shears$^{62}$\lhcborcid{0000-0002-2653-1366},
L.~Shekhtman$^{44}$\lhcborcid{0000-0003-1512-9715},
Z.~Shen$^{38}$\lhcborcid{0000-0003-1391-5384},
S.~Sheng$^{5,7}$\lhcborcid{0000-0002-1050-5649},
V.~Shevchenko$^{44}$\lhcborcid{0000-0003-3171-9125},
B.~Shi$^{7}$\lhcborcid{0000-0002-5781-8933},
Q.~Shi$^{7}$\lhcborcid{0000-0001-7915-8211},
W. S. ~Shi$^{74}$\lhcborcid{0009-0003-4186-9191},
Y.~Shimizu$^{14}$\lhcborcid{0000-0002-4936-1152},
E.~Shmanin$^{25}$\lhcborcid{0000-0002-8868-1730},
R.~Shorkin$^{44}$\lhcborcid{0000-0001-8881-3943},
J.D.~Shupperd$^{70}$\lhcborcid{0009-0006-8218-2566},
R.~Silva~Coutinho$^{2}$\lhcborcid{0000-0002-1545-959X},
G.~Simi$^{33,r}$\lhcborcid{0000-0001-6741-6199},
S.~Simone$^{24,i}$\lhcborcid{0000-0003-3631-8398},
M. ~Singha$^{81}$\lhcborcid{0009-0005-1271-972X},
N.~Skidmore$^{58}$\lhcborcid{0000-0003-3410-0731},
T.~Skwarnicki$^{70}$\lhcborcid{0000-0002-9897-9506},
M.W.~Slater$^{55}$\lhcborcid{0000-0002-2687-1950},
E.~Smith$^{66}$\lhcborcid{0000-0002-9740-0574},
K.~Smith$^{69}$\lhcborcid{0000-0002-1305-3377},
M.~Smith$^{63}$\lhcborcid{0000-0002-3872-1917},
L.~Soares~Lavra$^{60}$\lhcborcid{0000-0002-2652-123X},
M.D.~Sokoloff$^{67}$\lhcborcid{0000-0001-6181-4583},
F.J.P.~Soler$^{61}$\lhcborcid{0000-0002-4893-3729},
A.~Solomin$^{56}$\lhcborcid{0000-0003-0644-3227},
A.~Solovev$^{44}$\lhcborcid{0000-0002-5355-5996},
K. ~Solovieva$^{20}$\lhcborcid{0000-0003-2168-9137},
N. S. ~Sommerfeld$^{18}$\lhcborcid{0009-0006-7822-2860},
R.~Song$^{1}$\lhcborcid{0000-0002-8854-8905},
Y.~Song$^{51}$\lhcborcid{0000-0003-0256-4320},
Y.~Song$^{4,d}$\lhcborcid{0000-0003-1959-5676},
Y. S. ~Song$^{6}$\lhcborcid{0000-0003-3471-1751},
F.L.~Souza~De~Almeida$^{46}$\lhcborcid{0000-0001-7181-6785},
B.~Souza~De~Paula$^{3}$\lhcborcid{0009-0003-3794-3408},
K.M.~Sowa$^{40}$\lhcborcid{0000-0001-6961-536X},
E.~Spadaro~Norella$^{29,n}$\lhcborcid{0000-0002-1111-5597},
E.~Spedicato$^{25}$\lhcborcid{0000-0002-4950-6665},
J.G.~Speer$^{19}$\lhcborcid{0000-0002-6117-7307},
P.~Spradlin$^{61}$\lhcborcid{0000-0002-5280-9464},
F.~Stagni$^{50}$\lhcborcid{0000-0002-7576-4019},
M.~Stahl$^{80}$\lhcborcid{0000-0001-8476-8188},
S.~Stahl$^{50}$\lhcborcid{0000-0002-8243-400X},
S.~Stanislaus$^{65}$\lhcborcid{0000-0003-1776-0498},
M. ~Stefaniak$^{89}$\lhcborcid{0000-0002-5820-1054},
E.N.~Stein$^{50}$\lhcborcid{0000-0001-5214-8865},
O.~Steinkamp$^{52}$\lhcborcid{0000-0001-7055-6467},
D.~Strekalina$^{44}$\lhcborcid{0000-0003-3830-4889},
Y.~Su$^{7}$\lhcborcid{0000-0002-2739-7453},
F.~Suljik$^{65}$\lhcborcid{0000-0001-6767-7698},
J.~Sun$^{32}$\lhcborcid{0000-0002-6020-2304},
J. ~Sun$^{64}$\lhcborcid{0009-0008-7253-1237},
L.~Sun$^{76}$\lhcborcid{0000-0002-0034-2567},
D.~Sundfeld$^{2}$\lhcborcid{0000-0002-5147-3698},
W.~Sutcliffe$^{52}$\lhcborcid{0000-0002-9795-3582},
P.~Svihra$^{79}$\lhcborcid{0000-0002-7811-2147},
V.~Svintozelskyi$^{49}$\lhcborcid{0000-0002-0798-5864},
K.~Swientek$^{40}$\lhcborcid{0000-0001-6086-4116},
F.~Swystun$^{57}$\lhcborcid{0009-0006-0672-7771},
A.~Szabelski$^{42}$\lhcborcid{0000-0002-6604-2938},
T.~Szumlak$^{40}$\lhcborcid{0000-0002-2562-7163},
Y.~Tan$^{4}$\lhcborcid{0000-0003-3860-6545},
Y.~Tang$^{76}$\lhcborcid{0000-0002-6558-6730},
Y. T. ~Tang$^{7}$\lhcborcid{0009-0003-9742-3949},
M.D.~Tat$^{22}$\lhcborcid{0000-0002-6866-7085},
J. A.~Teijeiro~Jimenez$^{48}$\lhcborcid{0009-0004-1845-0621},
A.~Terentev$^{44}$\lhcborcid{0000-0003-2574-8560},
F.~Terzuoli$^{35,w}$\lhcborcid{0000-0002-9717-225X},
F.~Teubert$^{50}$\lhcborcid{0000-0003-3277-5268},
E.~Thomas$^{50}$\lhcborcid{0000-0003-0984-7593},
D.J.D.~Thompson$^{55}$\lhcborcid{0000-0003-1196-5943},
A. R. ~Thomson-Strong$^{60}$\lhcborcid{0009-0000-4050-6493},
H.~Tilquin$^{63}$\lhcborcid{0000-0003-4735-2014},
V.~Tisserand$^{11}$\lhcborcid{0000-0003-4916-0446},
S.~T'Jampens$^{10}$\lhcborcid{0000-0003-4249-6641},
M.~Tobin$^{5,50}$\lhcborcid{0000-0002-2047-7020},
T. T. ~Todorov$^{20}$\lhcborcid{0009-0002-0904-4985},
L.~Tomassetti$^{26,m}$\lhcborcid{0000-0003-4184-1335},
G.~Tonani$^{30}$\lhcborcid{0000-0001-7477-1148},
X.~Tong$^{6}$\lhcborcid{0000-0002-5278-1203},
T.~Tork$^{30}$\lhcborcid{0000-0001-9753-329X},
D.~Torres~Machado$^{2}$\lhcborcid{0000-0001-7030-6468},
L.~Toscano$^{19}$\lhcborcid{0009-0007-5613-6520},
D.Y.~Tou$^{4,d}$\lhcborcid{0000-0002-4732-2408},
C.~Trippl$^{47}$\lhcborcid{0000-0003-3664-1240},
G.~Tuci$^{22}$\lhcborcid{0000-0002-0364-5758},
N.~Tuning$^{38}$\lhcborcid{0000-0003-2611-7840},
L.H.~Uecker$^{22}$\lhcborcid{0000-0003-3255-9514},
A.~Ukleja$^{40}$\lhcborcid{0000-0003-0480-4850},
D.J.~Unverzagt$^{22}$\lhcborcid{0000-0002-1484-2546},
A. ~Upadhyay$^{50}$\lhcborcid{0009-0000-6052-6889},
B. ~Urbach$^{60}$\lhcborcid{0009-0001-4404-561X},
A.~Usachov$^{38}$\lhcborcid{0000-0002-5829-6284},
A.~Ustyuzhanin$^{44}$\lhcborcid{0000-0001-7865-2357},
U.~Uwer$^{22}$\lhcborcid{0000-0002-8514-3777},
V.~Vagnoni$^{25,50}$\lhcborcid{0000-0003-2206-311X},
A. ~Vaitkevicius$^{82}$\lhcborcid{0000-0003-3625-198X},
V. ~Valcarce~Cadenas$^{48}$\lhcborcid{0009-0006-3241-8964},
G.~Valenti$^{25}$\lhcborcid{0000-0002-6119-7535},
N.~Valls~Canudas$^{50}$\lhcborcid{0000-0001-8748-8448},
J.~van~Eldik$^{50}$\lhcborcid{0000-0002-3221-7664},
H.~Van~Hecke$^{69}$\lhcborcid{0000-0001-7961-7190},
E.~van~Herwijnen$^{63}$\lhcborcid{0000-0001-8807-8811},
C.B.~Van~Hulse$^{48,z}$\lhcborcid{0000-0002-5397-6782},
R.~Van~Laak$^{51}$\lhcborcid{0000-0002-7738-6066},
M.~van~Veghel$^{84}$\lhcborcid{0000-0001-6178-6623},
G.~Vasquez$^{52}$\lhcborcid{0000-0002-3285-7004},
R.~Vazquez~Gomez$^{46}$\lhcborcid{0000-0001-5319-1128},
P.~Vazquez~Regueiro$^{48}$\lhcborcid{0000-0002-0767-9736},
C.~V{\'a}zquez~Sierra$^{45}$\lhcborcid{0000-0002-5865-0677},
S.~Vecchi$^{26}$\lhcborcid{0000-0002-4311-3166},
J. ~Velilla~Serna$^{49}$\lhcborcid{0009-0006-9218-6632},
J.J.~Velthuis$^{56}$\lhcborcid{0000-0002-4649-3221},
M.~Veltri$^{27,x}$\lhcborcid{0000-0001-7917-9661},
A.~Venkateswaran$^{51}$\lhcborcid{0000-0001-6950-1477},
M.~Verdoglia$^{32}$\lhcborcid{0009-0006-3864-8365},
M.~Vesterinen$^{58}$\lhcborcid{0000-0001-7717-2765},
W.~Vetens$^{70}$\lhcborcid{0000-0003-1058-1163},
D. ~Vico~Benet$^{65}$\lhcborcid{0009-0009-3494-2825},
P. ~Vidrier~Villalba$^{46}$\lhcborcid{0009-0005-5503-8334},
M.~Vieites~Diaz$^{48}$\lhcborcid{0000-0002-0944-4340},
X.~Vilasis-Cardona$^{47}$\lhcborcid{0000-0002-1915-9543},
E.~Vilella~Figueras$^{62}$\lhcborcid{0000-0002-7865-2856},
A.~Villa$^{25}$\lhcborcid{0000-0002-9392-6157},
P.~Vincent$^{16}$\lhcborcid{0000-0002-9283-4541},
B.~Vivacqua$^{3}$\lhcborcid{0000-0003-2265-3056},
F.C.~Volle$^{55}$\lhcborcid{0000-0003-1828-3881},
D.~vom~Bruch$^{13}$\lhcborcid{0000-0001-9905-8031},
N.~Voropaev$^{44}$\lhcborcid{0000-0002-2100-0726},
K.~Vos$^{84}$\lhcborcid{0000-0002-4258-4062},
C.~Vrahas$^{60}$\lhcborcid{0000-0001-6104-1496},
J.~Wagner$^{19}$\lhcborcid{0000-0002-9783-5957},
J.~Walsh$^{35}$\lhcborcid{0000-0002-7235-6976},
E.J.~Walton$^{1,58}$\lhcborcid{0000-0001-6759-2504},
G.~Wan$^{6}$\lhcborcid{0000-0003-0133-1664},
A. ~Wang$^{7}$\lhcborcid{0009-0007-4060-799X},
B. ~Wang$^{5}$\lhcborcid{0009-0008-4908-087X},
C.~Wang$^{22}$\lhcborcid{0000-0002-5909-1379},
G.~Wang$^{8}$\lhcborcid{0000-0001-6041-115X},
H.~Wang$^{75}$\lhcborcid{0009-0008-3130-0600},
J.~Wang$^{7}$\lhcborcid{0000-0001-7542-3073},
J.~Wang$^{5}$\lhcborcid{0000-0002-6391-2205},
J.~Wang$^{4,d}$\lhcborcid{0000-0002-3281-8136},
J.~Wang$^{76}$\lhcborcid{0000-0001-6711-4465},
M.~Wang$^{50}$\lhcborcid{0000-0003-4062-710X},
N. W. ~Wang$^{7}$\lhcborcid{0000-0002-6915-6607},
R.~Wang$^{56}$\lhcborcid{0000-0002-2629-4735},
X.~Wang$^{8}$\lhcborcid{0009-0006-3560-1596},
X.~Wang$^{74}$\lhcborcid{0000-0002-2399-7646},
X. W. ~Wang$^{63}$\lhcborcid{0000-0001-9565-8312},
Y.~Wang$^{77}$\lhcborcid{0000-0003-3979-4330},
Y.~Wang$^{6}$\lhcborcid{0009-0003-2254-7162},
Y. H. ~Wang$^{75}$\lhcborcid{0000-0003-1988-4443},
Z.~Wang$^{14}$\lhcborcid{0000-0002-5041-7651},
Z.~Wang$^{30}$\lhcborcid{0000-0003-4410-6889},
J.A.~Ward$^{58,1}$\lhcborcid{0000-0003-4160-9333},
M.~Waterlaat$^{50}$\lhcborcid{0000-0002-2778-0102},
N.K.~Watson$^{55}$\lhcborcid{0000-0002-8142-4678},
D.~Websdale$^{63}$\lhcborcid{0000-0002-4113-1539},
Y.~Wei$^{6}$\lhcborcid{0000-0001-6116-3944},
Z. ~Weida$^{7}$\lhcborcid{0009-0002-4429-2458},
J.~Wendel$^{45}$\lhcborcid{0000-0003-0652-721X},
B.D.C.~Westhenry$^{56}$\lhcborcid{0000-0002-4589-2626},
C.~White$^{57}$\lhcborcid{0009-0002-6794-9547},
M.~Whitehead$^{61}$\lhcborcid{0000-0002-2142-3673},
E.~Whiter$^{55}$\lhcborcid{0009-0003-3902-8123},
A.R.~Wiederhold$^{64}$\lhcborcid{0000-0002-1023-1086},
D.~Wiedner$^{19}$\lhcborcid{0000-0002-4149-4137},
M. A.~Wiegertjes$^{38}$\lhcborcid{0009-0002-8144-422X},
C. ~Wild$^{65}$\lhcborcid{0009-0008-1106-4153},
G.~Wilkinson$^{65,50}$\lhcborcid{0000-0001-5255-0619},
M.K.~Wilkinson$^{67}$\lhcborcid{0000-0001-6561-2145},
M.~Williams$^{66}$\lhcborcid{0000-0001-8285-3346},
M. J.~Williams$^{50}$\lhcborcid{0000-0001-7765-8941},
M.R.J.~Williams$^{60}$\lhcborcid{0000-0001-5448-4213},
R.~Williams$^{57}$\lhcborcid{0000-0002-2675-3567},
S. ~Williams$^{56}$\lhcborcid{ 0009-0007-1731-8700},
Z. ~Williams$^{56}$\lhcborcid{0009-0009-9224-4160},
F.F.~Wilson$^{59}$\lhcborcid{0000-0002-5552-0842},
M.~Winn$^{12}$\lhcborcid{0000-0002-2207-0101},
W.~Wislicki$^{42}$\lhcborcid{0000-0001-5765-6308},
M.~Witek$^{41}$\lhcborcid{0000-0002-8317-385X},
L.~Witola$^{19}$\lhcborcid{0000-0001-9178-9921},
T.~Wolf$^{22}$\lhcborcid{0009-0002-2681-2739},
E. ~Wood$^{57}$\lhcborcid{0009-0009-9636-7029},
G.~Wormser$^{14}$\lhcborcid{0000-0003-4077-6295},
S.A.~Wotton$^{57}$\lhcborcid{0000-0003-4543-8121},
H.~Wu$^{70}$\lhcborcid{0000-0002-9337-3476},
J.~Wu$^{8}$\lhcborcid{0000-0002-4282-0977},
X.~Wu$^{76}$\lhcborcid{0000-0002-0654-7504},
Y.~Wu$^{6,57}$\lhcborcid{0000-0003-3192-0486},
Z.~Wu$^{7}$\lhcborcid{0000-0001-6756-9021},
K.~Wyllie$^{50}$\lhcborcid{0000-0002-2699-2189},
S.~Xian$^{74}$\lhcborcid{0009-0009-9115-1122},
Z.~Xiang$^{5}$\lhcborcid{0000-0002-9700-3448},
Y.~Xie$^{8}$\lhcborcid{0000-0001-5012-4069},
T. X. ~Xing$^{30}$\lhcborcid{0009-0006-7038-0143},
A.~Xu$^{35,t}$\lhcborcid{0000-0002-8521-1688},
L.~Xu$^{4,d}$\lhcborcid{0000-0002-0241-5184},
M.~Xu$^{50}$\lhcborcid{0000-0001-8885-565X},
Z.~Xu$^{50}$\lhcborcid{0000-0002-7531-6873},
Z.~Xu$^{7}$\lhcborcid{0000-0001-9558-1079},
Z.~Xu$^{5}$\lhcborcid{0000-0001-9602-4901},
S. ~Yadav$^{26}$\lhcborcid{0009-0007-5014-1636},
K. ~Yang$^{63}$\lhcborcid{0000-0001-5146-7311},
X.~Yang$^{6}$\lhcborcid{0000-0002-7481-3149},
Y.~Yang$^{7}$\lhcborcid{0000-0002-8917-2620},
Y. ~Yang$^{81}$\lhcborcid{0009-0009-3430-0558},
Z.~Yang$^{6}$\lhcborcid{0000-0003-2937-9782},
V.~Yeroshenko$^{14}$\lhcborcid{0000-0002-8771-0579},
H.~Yeung$^{64}$\lhcborcid{0000-0001-9869-5290},
H.~Yin$^{8}$\lhcborcid{0000-0001-6977-8257},
X. ~Yin$^{7}$\lhcborcid{0009-0003-1647-2942},
C. Y. ~Yu$^{6}$\lhcborcid{0000-0002-4393-2567},
J.~Yu$^{73}$\lhcborcid{0000-0003-1230-3300},
X.~Yuan$^{5}$\lhcborcid{0000-0003-0468-3083},
Y~Yuan$^{5,7}$\lhcborcid{0009-0000-6595-7266},
J. A.~Zamora~Saa$^{72}$\lhcborcid{0000-0002-5030-7516},
M.~Zavertyaev$^{21}$\lhcborcid{0000-0002-4655-715X},
M.~Zdybal$^{41}$\lhcborcid{0000-0002-1701-9619},
F.~Zenesini$^{25}$\lhcborcid{0009-0001-2039-9739},
C. ~Zeng$^{5,7}$\lhcborcid{0009-0007-8273-2692},
M.~Zeng$^{4,d}$\lhcborcid{0000-0001-9717-1751},
C.~Zhang$^{6}$\lhcborcid{0000-0002-9865-8964},
D.~Zhang$^{8}$\lhcborcid{0000-0002-8826-9113},
J.~Zhang$^{7}$\lhcborcid{0000-0001-6010-8556},
L.~Zhang$^{4,d}$\lhcborcid{0000-0003-2279-8837},
R.~Zhang$^{8}$\lhcborcid{0009-0009-9522-8588},
S.~Zhang$^{73}$\lhcborcid{0000-0002-9794-4088},
S.~Zhang$^{65}$\lhcborcid{0000-0002-2385-0767},
Y.~Zhang$^{6}$\lhcborcid{0000-0002-0157-188X},
Y. Z. ~Zhang$^{4,d}$\lhcborcid{0000-0001-6346-8872},
Z.~Zhang$^{4,d}$\lhcborcid{0000-0002-1630-0986},
Y.~Zhao$^{22}$\lhcborcid{0000-0002-8185-3771},
A.~Zhelezov$^{22}$\lhcborcid{0000-0002-2344-9412},
S. Z. ~Zheng$^{6}$\lhcborcid{0009-0001-4723-095X},
X. Z. ~Zheng$^{4,d}$\lhcborcid{0000-0001-7647-7110},
Y.~Zheng$^{7}$\lhcborcid{0000-0003-0322-9858},
T.~Zhou$^{6}$\lhcborcid{0000-0002-3804-9948},
X.~Zhou$^{8}$\lhcborcid{0009-0005-9485-9477},
Y.~Zhou$^{7}$\lhcborcid{0000-0003-2035-3391},
V.~Zhovkovska$^{58}$\lhcborcid{0000-0002-9812-4508},
L. Z. ~Zhu$^{7}$\lhcborcid{0000-0003-0609-6456},
X.~Zhu$^{4,d}$\lhcborcid{0000-0002-9573-4570},
X.~Zhu$^{8}$\lhcborcid{0000-0002-4485-1478},
Y. ~Zhu$^{17}$\lhcborcid{0009-0004-9621-1028},
V.~Zhukov$^{17}$\lhcborcid{0000-0003-0159-291X},
J.~Zhuo$^{49}$\lhcborcid{0000-0002-6227-3368},
Q.~Zou$^{5,7}$\lhcborcid{0000-0003-0038-5038},
D.~Zuliani$^{33,r}$\lhcborcid{0000-0002-1478-4593},
G.~Zunica$^{28}$\lhcborcid{0000-0002-5972-6290}.\bigskip

{\footnotesize \it

$^{1}$School of Physics and Astronomy, Monash University, Melbourne, Australia\\
$^{2}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{3}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{4}$Department of Engineering Physics, Tsinghua University, Beijing, China\\
$^{5}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{6}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{7}$University of Chinese Academy of Sciences, Beijing, China\\
$^{8}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{9}$Consejo Nacional de Rectores  (CONARE), San Jose, Costa Rica\\
$^{10}$Universit{\'e} Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{11}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{12}$Universit{\'e} Paris-Saclay, Centre d'Etudes de Saclay (CEA), IRFU, Saclay, France, Gif-Sur-Yvette, France\\
$^{13}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{14}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{15}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{16}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{17}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{18}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany\\
$^{19}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{20}$Physikalisches Institut, Albert-Ludwigs-Universit{\"a}t Freiburg, Freiburg, Germany\\
$^{21}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{22}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{23}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{24}$INFN Sezione di Bari, Bari, Italy\\
$^{25}$INFN Sezione di Bologna, Bologna, Italy\\
$^{26}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{27}$INFN Sezione di Firenze, Firenze, Italy\\
$^{28}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{29}$INFN Sezione di Genova, Genova, Italy\\
$^{30}$INFN Sezione di Milano, Milano, Italy\\
$^{31}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{32}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{33}$INFN Sezione di Padova, Padova, Italy\\
$^{34}$INFN Sezione di Perugia, Perugia, Italy\\
$^{35}$INFN Sezione di Pisa, Pisa, Italy\\
$^{36}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{37}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{38}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{39}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{40}$AGH - University of Krakow, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{41}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{42}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{43}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{44}$Authors affiliated with an institute formerly covered by a cooperation agreement with CERN.\\
$^{45}$Universidade da Coru{\~n}a, A Coru{\~n}a, Spain\\
$^{46}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{47}$La Salle, Universitat Ramon Llull, Barcelona, Spain\\
$^{48}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{49}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{50}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{51}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{52}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{53}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{54}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{55}$School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{56}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{57}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{58}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{59}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{60}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{61}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{62}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{63}$Imperial College London, London, United Kingdom\\
$^{64}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{65}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{66}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{67}$University of Cincinnati, Cincinnati, OH, United States\\
$^{68}$University of Maryland, College Park, MD, United States\\
$^{69}$Los Alamos National Laboratory (LANL), Los Alamos, NM, United States\\
$^{70}$Syracuse University, Syracuse, NY, United States\\
$^{71}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{3}$\\
$^{72}$Universidad Andres Bello, Santiago, Chile, associated to $^{52}$\\
$^{73}$School of Physics and Electronics, Hunan University, Changsha City, China, associated to $^{8}$\\
$^{74}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{4}$\\
$^{75}$Lanzhou University, Lanzhou, China, associated to $^{5}$\\
$^{76}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{4}$\\
$^{77}$Henan Normal University, Xinxiang, China, associated to $^{8}$\\
$^{78}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{16}$\\
$^{79}$Institute of Physics of  the Czech Academy of Sciences, Prague, Czech Republic, associated to $^{64}$\\
$^{80}$Ruhr Universitaet Bochum, Fakultaet f. Physik und Astronomie, Bochum, Germany, associated to $^{19}$\\
$^{81}$Eotvos Lorand University, Budapest, Hungary, associated to $^{50}$\\
$^{82}$Faculty of Physics, Vilnius University, Vilnius, Lithuania, associated to $^{20}$\\
$^{83}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{38}$\\
$^{84}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{38}$\\
$^{85}$Tadeusz Kosciuszko Cracow University of Technology, Cracow, Poland, associated to $^{41}$\\
$^{86}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{61}$\\
$^{87}$Taras Schevchenko University of Kyiv, Faculty of Physics, Kyiv, Ukraine, associated to $^{14}$\\
$^{88}$University of Michigan, Ann Arbor, MI, United States, associated to $^{70}$\\
$^{89}$Ohio State University, Columbus, United States, associated to $^{69}$\\
\bigskip
$^{a}$Universidade Estadual de Campinas (UNICAMP), Campinas, Brazil\\
$^{b}$Centro Federal de Educac{\~a}o Tecnol{\'o}gica Celso Suckow da Fonseca, Rio De Janeiro, Brazil\\
$^{c}$Department of Physics and Astronomy, University of Victoria, Victoria, Canada\\
$^{d}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{e}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{f}$LIP6, Sorbonne Universit{\'e}, Paris, France\\
$^{g}$Lamarr Institute for Machine Learning and Artificial Intelligence, Dortmund, Germany\\
$^{h}$Universidad Nacional Aut{\'o}noma de Honduras, Tegucigalpa, Honduras\\
$^{i}$Universit{\`a} di Bari, Bari, Italy\\
$^{j}$Universit{\`a} di Bergamo, Bergamo, Italy\\
$^{k}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{l}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{m}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{n}$Universit{\`a} di Genova, Genova, Italy\\
$^{o}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{p}$Universit{\`a} degli Studi di Milano-Bicocca, Milano, Italy\\
$^{q}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{r}$Universit{\`a} di Padova, Padova, Italy\\
$^{s}$Universit{\`a}  di Perugia, Perugia, Italy\\
$^{t}$Scuola Normale Superiore, Pisa, Italy\\
$^{u}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{v}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{w}$Universit{\`a} di Siena, Siena, Italy\\
$^{x}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{y}$Universidad de Ingenier\'{i}a y Tecnolog\'{i}a (UTEC), Lima, Peru\\
$^{z}$Universidad de Alcal{\'a}, Alcal{\'a} de Henares , Spain\\
\medskip
}
\end{flushleft}
